ISO-SWS calibration and the accurate modelling of cool-star atmospheres - IV. G9 to M2 stars

presented. The 2.38 -- 4.08 micron wavelength-range of band 1 of ISO-SWS (Short-Wavelength Spectrometers on board of the Infrared Space Observatory) in which many different molecules -- with their own dependence on each of the stellar parameters -- are absorbing, enables us to estimate the effective temperature, the gravity, the microturbulence, the metallicity, the CNO-abundances, the 12C/13C-ratio and the angular diameter from the ISO-SWS data. Using the Hipparcos' parallax, the radius, luminosity and gravity-inferred mass are derived. The stellar parameters obtained are in good agreement with other published values, though also some discrepancies with values deduced by other authors are noted. For a few stars (Delta Dra, Xi Dra, Alpha Tuc, H Sco and Alpha Cet) some parameters -- e.g. the CNO-abundances -- are derived for the first time. By examining the correspondence between different ISO-SWS observations of the same object and between the ISO-SWS data and the corresponding synthetic spectrum, it is shown that the relative accuracy of ISO-SWS in band 1 (2.38 -- 4.0 micron) is better than 2% for these high-flux sources. The high level of correspondence between observations and theoretical predictions, together with a confrontation of the estimated Teff(ISO) value with Teff-values derived from colours -- which demonstrates the consistency between V-K, BC(K), Teff and the angular diameter derived from optical or IR data -- proves that both the used MARCS models to derive the stellar quantities and the flux calibration of the ISO-SWS detectors have reached a high level of reliability.

==> h3319_mac.tex <==
%% file: rrmacros2e.tex = Rob Rutten's standard LaTeX macros
%% last: Apr 20 2000
%% site: ~/rr/dip/texdip

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% BIBTEX EXPLANATION
%% Use BibTeX with the proper JOURNAL.STY, BIB.STY and BIB.BST style files.
%% The required statement combinations sit in template files:
%%    RRPAPER.TPL, AAPAPER.TPL, APJPAPER.TPL, ESAPROC.TPL, KLUWER.TPL,
%%    SWANSONG.TPL, PASP.TPL etc.,  
%% linked to directory /rrtex/templates
%% My RJR-typed -.BIB files are linked to /rrtex/bibfiles/rjr/bib.
%% My ADS-copied -.BIB files are linked to /rrtex/bibfiles/ads/bib.
%% Journal abbreviations are specified in AAJOUR.BIB (A&A, APJ format) and
%%   in JOURNALS.BIB (classical longer format), both in /rrtex/styles.
%%   The ADS abbreviations are redefined below (also two formats).
%% To use bibtex use script rrbibtex (in ~rutten/bin).
%%
%% Cites:   \cite*{Rutten1990a}                        }      
%%               ==>  Rutten (1990)                    } for in-text
%%          \cite*{Gurtovenko+Kostik+Rutten1990b}      } references
%%               ==>  Gurtovenko et al. (1990)        }
%%          \cite{Rutten1990a}                       }
%%               ==>  Rutten 1990                    } for between (...)
%%          \cite{Gurtovenko+Kostik+Rutten1990b}     } references
%%               ==>  Gurtovenko et al. 1990          }
%%          (Rutten 1990a, 1990b)
%%                    \nocite{Rutten1990c}  
%%                    \nocite{Rutten1990f}
%%          NB: \nocite*{..} makes Bibtex produce ALL bibliography entries
%%          NB: Bibtex may mix up the order, putting a later paper
%%              before an earlier one even in the same journal, becauses it
%%              alphabetizes on title after authors.  If it bothers you
%%              then correct the final -.BBL file, or fix the problem
%%              by adding fake digits to TITLE fields in .BIB files 
%%              (see Jo Bruls' README_order with my -.BIB files).
%%
%% Full citations for publication lists and PRINTBIB:
%%              \fullreferences (adds full titles and end pages)
%% 
%% References:
%%          - RRBIB: \section*{References} \references 
%%          - FULLBIB: \section*{References} \fullreferences
%%          - AABIB: no section header, \aareferences
%%          - APJBIB: no section header, \apjreferences
%%          - KLUWBIB: no section header, \references
%%          - ESA: no BIB.STY, section header ESAPROC.TPL, \esareferences
%%          - set \parsep=0ex to delete blank lines between references
%%          - execute latex, rrbibtex, latex twice
%%          - for email/ftp transfer: comment \references statement out and
%%            merge the -.BBL file there instead, or ftp that as well.
%%            Also ftp or insert this macro file, and email/ftp xxxBIB.STY.
%%
%% Database printout: ps files under /rrtex/bibfiles
%%
%% ADS: As of July 1996 I use ADS entries.  I  pull XXX.BIB files over
%%      from ADS and also XXX.ABS files with the corresponding abstracts.  
%%      They sit in /rrtex/bibfiles/ads/bib and /rrtex/bibfiles/ads/abs.
%%      Script RRBIBTEX copies all the XXX.BIB files to a short-lived
%%      file /scratch/strknd/rutten/adsfiles.bib that is searched by BibTeX 
%%      (appropriate BibTeX path in my .login) from script RRBIBTEX.
%%      BibTeX may complain about repeated ADS entries; don't bother.
%% NB: don't refer to the same paper with both its ADS XXX.BIB label 
%%     and its old bibfile label - or you get that reference twice.
%%     Check the resulting reference list for such duplicates.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% ADS journal abbreviations: long and short versions, also in RJR.BIB
\newcount\longrefs
\def\aap{\ifnum\longrefs=1 {Astron.\ Astrophys.}\else 
                           {A\hbox{\rm \&}A}\fi}
\def\aapr{\ifnum\longrefs=1 {Astron.\ Astrophys.\ Rev.}\else 
                            {A\hbox{\rm \&}AR}\fi}
\def\aaps{\ifnum\longrefs=1 {Astron.\ Astrophys.\ Suppl.}\else 
                            {A\hbox{\rm \&}AS}\fi}
\def\aj{\ifnum\longrefs=1 {Astron.\ J.}\else 
                          {AJ}\fi} 
\def\ao{\ifnum\longrefs=1 {Applied Optics}\else 
                           {Appl.\ Opt.}\fi} 
\def\aspcs{\ifnum\longrefs=1 {Astron.\ Soc.\ Pacific Conf. Series}\else 
                           {ASP Conf.\ Ser.}\fi} 
\def\apj{\ifnum\longrefs=1 {Astrophys.\ J.}\else 
                           {ApJ}\fi} 
\def\apjl{\ifnum\longrefs=1 {Astrophys.\ J. Lett.}\else 
                            {ApJ}\fi} 
\def\aplett{\ifnum\longrefs=1 {Astrophys.\ J. Lett.}\else 
                            {ApJ}\fi} 
\def\apjs{\ifnum\longrefs=1 {Astrophys.\ J. Suppl.}\else 
                            {ApJS}\fi}
\def\apss{\ifnum\longrefs=1 {Astrophys.\ and Space Science}\else 
                            {Ap\hbox{\rm \&}SS}\fi}
\def\araa{\ifnum\longrefs=1 {Ann.\ Rev.\ Astron.\ Astrophys.}\else 
                            {ARA\hbox{\rm \&}A}\fi}
\def\azh{\ifnum\longrefs=1 {Astronomicheskii Zhurnal}\else 
                            {Astron.\ Zhur.}\fi}
\def\baas{\ifnum\longrefs=1 {Bull.\ Am.\ Astron.\ Soc.}\else 
                            {BAAS}\fi}
\def\bain{\ifnum\longrefs=1 {Bull.\ Astronom.\ Institutes Netherlands}\else
                            {Bull.\ Astr.\ Inst.\ Neth.}\fi}
\def\gca{\ifnum\longrefs=1 {Geochim.\ Cosmochim.\ Acta}\else 
                           {Geochim.\ Cosmochim.\ Acta}\fi}
\def\grl{\ifnum\longrefs=1 {Geophys.\ Res.\ Lett.}\else 
                           {Geoph.\ Res.\ Lett.}\fi}
\def\iaucirc{\ifnum\longrefs=1 {IAU Circulars}\else 
                          {IAU Circ.}\fi}
\def\ip{\ifnum\longrefs=1 {in press}\else 
                          {in press}\fi}
\def\jgr{\ifnum\longrefs=1 {J.\ Geophys.\ Res.}\else 
                           {J.\ Geophys.\ Res.}\fi}  
\def\jrasc{\ifnum\longrefs=1 {J.\ Royal Astron.\ Soc.\ Canada}\else 
                           {JRAS Can.}\fi}  
\def\mnras{\ifnum\longrefs=1 {Mon.\ Not.\ Roy.\ Astron.\ Soc.}\else 
                             {MNRAS}\fi} 
\def\nat{\ifnum\longrefs=1 {Nature}\else 
                           {Nat}\fi}
\def\pasj{\ifnum\longrefs=1 {Pub.\ Astron.\ Soc.\ Japan}\else 
                            {PASJ}\fi} 
\def\pasp{\ifnum\longrefs=1 {Pub.\ Astron.\ Soc.\ Pacific}\else 
                            {PASP}\fi} 
\def\physscr{\ifnum\longrefs=1 {Physica Scripta}\else 
                            {Phys.\ Scrip.}\fi} 
\def\planss{\ifnum\longrefs=1 {Planetary \& Space Science}\else 
                            {Plan. \& Space Sci.}\fi} 
\def\procspie{\ifnum\longrefs=1 {Proc.\ SPIE}\else 
                            {Proc.\ SPIE}\fi} 
\def\qjras{\ifnum\longrefs=1 {Quarterly J.\ Royal Astron.\ Soc.}\else 
                            {QJRAS}\fi} 
\def\sa{\ifnum\longrefs=1 {Soviet Astron..}\else 
                               {Sov.\ Astron.}\fi}
\def\skytel{\ifnum\longrefs=1 {Sky \& Telescope}\else 
                            {Sky \& Tel.}\fi} 
\def\solphys{\ifnum\longrefs=1 {Solar Phys.}\else 
                               {Solar Phys.}\fi}
\def\ssr{\ifnum\longrefs=1 {Space Science Rev.}\else 
                               {Space\ Sci.\ Rev.}\fi}

%% bibfile specification
%\def\bibfiles{/home/leen/latex/bibtex/bibliofile}   %% bibfiles

%% \references (JOURNALS.BIB and AAJOUR.BIB sit in /rrtex/styles)
%\def\references{\longrefs=1  \bibliographystyle{/home/leen/latex/bibtex/rrbib}
%             \bibliography{/home/leen/latex/bibtex/journals,\bibfiles}}
%\def\aareferences{\longrefs=0  \bibliographystyle{/home/leen/latex/bibtex/aa}
%            \bibliography{/home/leen/latex/bibtex/aajour,\bibfiles}}
%\def\apjreferences{\longrefs=0  \bibliographystyle{/home/leen/latex/bibtex/apjbib}
%             \bibliography{/home/leen/latex/bibtex/ajour,\bibfiles}}
%\def\fullreferences{\longrefs=1  \bibliographystyle{/home/leen/latex/bibtex/namebib}
%             \bibliography{/home/leen/latex/bibtex/journals,\bibfiles}}
%\def\nlreferences{\longrefs=1  \bibliographystyle{/home/leen/latex/bibtex/nlbib}
%             \bibliography{/home/leen/latex/bibtex/journals,\bibfiles}}
%\def\titlereferences{\longrefs=1  \bibliographystyle{/home/leen/latex/bibtex/titlebib}
%             \bibliography{/home/leen/latex/bibtex/journals,\bibfiles}}
%\def\esareferences{\longrefs=1  \bibliographystyle{/home/leen/latex/bibtex/esabib} 
%             \bibliography{/home/leen/latex/bibtex/journals,\bibfiles}}
%\def\kluwreferences{\longrefs=1 \bibliographystyle{/home/leen/latex/bibtex/kluwbib}
%             \bibliography{/home/leen/latex/bibtex/journals,\bibfiles}}
%\def\kluwtitlereferences{\longrefs=1 \bibliographystyle{/home/leen/latex/bibtex/kluwtbib}
%             \bibliography{/home/leen/latex/bibtex/journals,\bibfiles}}
%\def\natbibreferences{\longrefs=1 \bibliographystyle{/home/leen/latex/bibtex/natbib/plainnat}
%             \bibliography{/home/leen/latex/bibtex/journals,\bibfiles}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% INSTITUTE ADDRESS ABBREVIATIONS
\def\nl{,\ } %%\def\nl{\newline}  %% redefine as \newline for mail addresses
\def\AFGL{Air Force Geophysics Lab.\nl Sunspot NM~88349\nl USA}
\def\Arcetri{Osservatorio Astrofisico di Arcetri\nl Largo E. Fermi 5\nl
         I--50125 Firenze\nl Italy}
\def\Armagh{Armagh Observatory\nl College Hill\nl Armagh, BT61~9DG\nl
         Northern Ireland}
\def\ASTRON{Stichting ASTRON\nl Postbus 2\nl NL--7990~AA Dwingeloo\nl
         The Netherlands}
\def\Caltech{Solar Astronomy\nl 105--24 Caltech\nl 
         Pasadena, CA~91125\nl USA}
\def\Catania{Osservatorio Astrofisico di Catania\nl Viale A. Doria 6\nl 
         Citta Universitaria\nl I--95125 Catania\nl Italy}
\def\CfA{Center for Astrophysics\nl 60 Garden Street\nl 
         Cambridge, MA~02138\nl USA}
\def\CHEAF{CHEAF\nl Kruislaan 403\nl NL--1098~SJ Amsterdam}
\def\DAMTP{Dept.\ Applied Math.\ and Theor.\ Phys.\nl Silver Street\nl 
         Cambridge CB3~9EW\nl United Kingdom}
\def\Dwingeloo{Radio Sterrewacht Dwingeloo\nl Postbus 2\nl
      NL--7990 AA Dwingeloo\nl The Netherlands}
\def\ESA{European Space Agency\nl 8--10 Rue Mario Nikis\nl
         F--75738 Paris Cedex 15\nl France} 
\def\ESO{European Southern Observatory\nl Karl--Schwarzschild-Str. 2\nl 
         D--85748 Garching bei M\"unchen\nl Germany}
\def\ESTEC{ESA Space Science Department\nl ESTEC\nl 
         Postbus 299\nl NL--2200~AG Noordwijk\nl The Netherlands}
\def\ETH{Institute of Astronomy\nl ETH--Zentrum\nl 
         CH--8092 Z\"urich\nl Switzerland}
\def\Goddard{NASA Goddard Space Flight Center \nl Greenbelt, MD~20771\nl USA}
\def\Goettingen{Universit\"{a}ts Sternwarte\nl Geismarlandstrasse 11\nl
         D--37083 G\"{o}ttingen\nl Germany}
\def\HAO{High Altitude Observatory\nl NCAR\nl PO Box 3000\nl 
         Boulder, CO 80307--3000\nl USA}
\def\Hawaii{Institute for Astronomy\nl 2680 Woodlawn Drive\nl 
         Honolulu, HAWAII 96822\nl USA}
\def\IAC{Instituto de Astrof{\'{\i}}sica de Canarias\nl C/ Via Lactea S/N\nl
         E--38200 La Laguna, Tenerife\nl Spain}
\def\IAP{Institut d'Astrophysique de Paris\nl 98-bis Boulevard Arago\nl
         F--75014 Paris\nl France}
\def\JILA{Joint Inst.\ Lab.\ Astrophysics\nl Campus Box 440\nl 
         Univ.\ Colorado\nl Boulder CO 80309--0440\nl USA}
\def\JPL{Jet Propulsion Laboratory\nl 4800 Oak Grove Drive\nl
         Pasadena CA~91109\nl USA}
\def\Kiel{Institut f\"ur Theor.\ Physik und Sternwarte\nl 
         Olshausenstrasse 40\nl D--2300 Kiel 1\nl Germany}  %% postcode?
\def\Kiev{Main Astronomical Observatory\nl Academy of Sciences Ukraine\nl 
         Golosiiv\nl  Kyiv 22\nl  252650 Ukraine}
\def\KIS{Kiepenheuer Institut f\"ur Sonnenphysik\nl Sch\"oneckstrasse 6\nl
         D--79104 Freiburg\nl Germany} 
\def\KSW{Kapteyn Sterrewacht\nl Mensingheweg 20\nl NL--9301 KA Roden\nl
         The Netherlands} 
\def\LKBF{Secretaris/Pennningmeester LKBF\nl \RUL}
\def\LPARL{Lockheed Martin ATC\nl Solar \& Astrophysics Lab\nl 
         Org.\ H1--12, Bldg.\ 252\nl 3251 Hanover Street\nl 
         Palo Alto, CA~94304--1187\nl USA}
\def\Meudon{Observatoire de Paris\nl F--92195 Meudon Principal Cedex\nl 
         France}
\def\NJIT{Department of Physics and Mathematics\nl
          New Jersey Institute of Technology\nl University Heights\nl
          Newark NJ 07102\nl USA}
\def\NOAO{National Opt.\ Astron.\ Obs.\nl P.O. Box 26732\nl 
         Tucson AZ 85726--26732\nl USA}
\def\NRL{Naval Research Laboratory\nl 
         Washington DC 20376--5000\nl USA}   %?? code
\def\NSO{National Solar Observatory\nl PO Box 26732\nl 
         Tucson AZ 85726--6732\nl USA}       
\def\Orsay{Institute d'Astrophysique Spatiale\nl 
         Universit\'e Paris XI--CNRS\nl B\^atiment 121\nl 
         F--91405 Orsay\nl France}
\def\Oslo{Institute of Theoretical Astrophysics\nl 
         P.O. Box 1029, Blindern\nl N--0315 Oslo\nl Norway}  
\def\OAC{Osservatorio di Capodimonte\nl Via Moiariello 16\nl 
         I--80131 Napoli\nl Italy}
\def\Ondrejov{Astronomical Institute\nl CS--25165 Ondrejov\nl Czech Republic}
\def\Potsdam{Astrophysikalisches Institut\nl Sonnenobservatorium 
         Einsteinturm\nl Telegrafenberg\nl D--14473 Potsdam\nl Germany}
\def\Pulkovo{Pulkovo Observatory\nl Pulskoske Shsee 65--1\nl
         196140 St.\ Petersburg\nl Russia}
\def\RUG{Kapteijn Laboratorium\nl Postbus 800\nl NL--9700~AV Groningen\nl
         The Netherlands}
\def\RUL{Sterrewacht\nl Postbus 9513\nl NL--2300~RA Leiden\nl 
         The Netherlands}
\def\SIU{Sterrekundig Instituut\nl Postbus 80\,000\nl
         NL--3508 TA Utrecht\nl The Netherlands}
\def\SPO{NSO/Sacramento Peak\nl P.O. Box 62\nl 
         Sunspot, NM 88349--0062\nl USA}
\def\Stanford{Center for Space Science and Astrophysics\nl  ERL 328\nl 
         Stanford University\nl Stanford CA 94305--4055\nl  USA}
\def\SRON{SRON\nl Sorbonnelaan 2\nl NL--3584 CA Utrecht\nl The Netherlands}
\def\SRONRUG{SRON\nl Postbus 800\nl NL--9700~AV Groningen\nl 
         The Netherlands}
\def\Uppsala{Astronomiska Observatoriet\nl Box 515\nl S--75120 Uppsala\nl
         Sweden}
\def\UvA{Sterrekundig Instituut ``Anton Pannekoek''\nl Kruislaan 403\nl
         NL--1098~SJ Amsterdam\nl The Netherlands}
\def\VU{Afdeling Sterrekunde\nl Vrije Universiteit\nl De Boelelaan 1081\nl
         NL--1081 HV Amsterdam\nl The Netherlands}
\def\Wuerzburg{Institut f\"ur Astronomie und Astrophysik\nl  Am Hubland\nl
      D--97074 W\"{u}rzburg\nl Germany}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% from DUTCH.STY
\def\dutch{\def\refname{Referenties}\def\abstractname{Samenvatting}%
  \def\bibname{Bibliografie}\def\chaptername{Hoofdstuk}%
  \def\appendixname{Bijlage}\def\contentsname{Inhoudsopgave}%
  \def\listfigurename{Lijst van figuren}\def\listtablename{Lijst van tabellen}%
  \def\indexname{Index}\def\figurename{Figuur}\def\tablename{Tabel}%
  \def\partname{Deel}\def\enclname{Bijlage(n)}\def\ccname{Ter attentie van}%
  \def\headtoname{Aan}\def\headpagename{Pagina}%
  \def\today{\number\day\space\ifcase\month\or januari\or februari\or maart\or%
     april\or mei\or juni\or juli\or augustus\or september\or oktober\or%
     november\or december\fi \space\number\year}%
  \typeout{
              >>>>> use hlatex209 for Dutch hyphenation <<<<< 
         }}
\hyphenation{Schrij-ver Krij-ger Kuij-pers Bal-le-gooij-en}
 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% warningoverprint
%% eg: \warningoverprint{DRAFT}, or SUBMITTED, CONFIDENTIAL from Eric Bakker
\def\warningoverprint #1{\special{!userdict begin 
  /bop-hook{gsave 100 600 translate -45 rotate /Times-Roman findfont 
  100 scalefont setfont 0 0 moveto 0.9 setgray (#1) show grestore}def end}}
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% figures
%% journal figures, use templettes in AAFIGS.TPL, APJFIGS.TPL, MULTIFIG.TPL
\newcounter{onefig} \newcounter{fignumber}
\newcount\nocaptions \newcount\nofigures \newcount\figwidth
\newcount\viewgraphs
\def\figsfile{} \def\figspath{} \def\paper{} \def\format{} \def\figlabel{} 
\long\def\nextfig#1{\setcounter{figure}{\value{fignumber}}
  \addtocounter{fignumber}{1}
  \ifnum \viewgraphs=1 \newpage \pagestyle{empty} \fi 
  \ifnum\value{onefig}=0 #1 \fi                 
  \ifnum\value{onefig}=\value{fignumber} #1 \fi}
\def\figwidths#1#2{\ifnum \nocaptions=1 #2mm \else #1mm \fi}  
%%\def\capspace#1{\vspace{#1}}     %% A&A: redefine \capspace = \picplace{#1}
\def\paper#1{}  %% redefine for separate-figure identification line
\long\def\plotfig#1#2{\ifnum \nofigures=1 \else #2 \fi}
\long\def\captiontext#1{\ifnum \nofigures=1 \raggedright \fi 
   \ifnum \nocaptions=1 \paper
     \ifnum \viewgraphs=0 
       \newline  \mbox{}\hrulefill\mbox{} \newline 
       \newline label:~\{\figlabel\} 
     \fi 
%%   \else \ifnum \nofigures=0 \{\figlabel\}~~ \fi   %% adds label
     \else \ifnum \nofigures=0 \fi 
   #1 \fi}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MULTI-FILE FIGURE
%% macros to combine separate postscript files into one multi-panel figure;
%% templettes in template files AAFIGS.TPL, APJFIGS.TPL, MULTIFIG.TPL.
%% - measure panel bounding boxes with GHOSTVIEW
%%   - large lower-left (outside axis labels)
%%   - small lower-left (between labels and numbers or just outside frame)
%%   - upper-left
%% - use \barepanel, \labelxpanel, \labelypanel, \labelxypanel 
%%   to control layout, for example to cut all x labels off and replace
%%   by single full-width LaTeX x label.  See templettes or test files.
%%   First specify \panelsize; \panelheight=0 maintains frame aspect ratio.
\newcount\panelwidth \newcount\panelheight 
\newcount\bxmin \newcount\bymin \newcount\bxmax \newcount\bymax
\newcount\tbxmin \newcount\tbymin
\newcount\tpanelwidth \newcount\tpanelheight \newcount\tpdif
\panelwidth=70 \panelheight=70  %% defaults (mm)
\def\panelsize #1,#2;{\panelwidth=#1 \panelheight=#2}  
     %% units MUST be mm; \panelheight=0 maintains frame aspect ratio
\def\setbb #1,#2;#3,#4;#5,#6;{% UNITS: bp (from ghostview)
  \tbxmin=#1 \tbymin=#2    %% full box (axis titles) lower left corner
  \bxmin=#3 \bymin=#4      %% bare box (ticks only) lower left corner
  \bxmax=#5 \bymax=#6}     %% upper right corner
\def\barepanel #1{%
  \ifnum\panelheight=0 
    \tpdif=\bymax \advance\tpdif by -\bymin
    \multiply \tpdif by \panelwidth
    \tpanelheight=\tpdif
    \tpdif=\bxmax \advance\tpdif by -\bxmin
    \divide \tpanelheight by \tpdif
  \else \tpanelheight=\panelheight \fi
  \epsfig{file=#1,%
     bbllx=\bxmin bp,bblly=\bymin bp,bburx=\bxmax bp,bbury=\bymax bp,clip=,%
     width=\panelwidth mm,height=\tpanelheight mm}}
\def\labelypanel #1{% TeX permits only integer arithmetic, so bp and mm
  \ifnum\panelheight=0 
    \tpdif=\bymax \advance\tpdif by -\bymin
    \multiply \tpdif by \panelwidth
    \tpanelheight=\tpdif
    \tpdif=\bxmax \advance\tpdif by -\bxmin
    \divide \tpanelheight by \tpdif
  \else \tpanelheight=\panelheight \fi
  \tpdif=\bxmax \advance\tpdif by -\tbxmin
  \tpanelwidth=\panelwidth \multiply \tpanelwidth by \tpdif
  \tpdif=\bxmax \advance\tpdif by -\bxmin
  \divide \tpanelwidth by \tpdif
  \epsfig{file=#1,%
    bbllx=\tbxmin bp,bblly=\bymin bp,bburx=\bxmax bp,bbury=\bymax bp,%
    clip=,width=\tpanelwidth mm,height=\tpanelheight mm}}
\def\labelxpanel #1{%
  \ifnum\panelheight=0 
    \tpdif=\bymax \advance\tpdif by -\bymin
    \multiply \tpdif by \panelwidth
    \tpanelheight=\tpdif
    \tpdif=\bxmax \advance\tpdif by -\bxmin
    \divide \tpanelheight by \tpdif
  \else \tpanelheight=\panelheight \fi
  \tpdif=\bymax \advance\tpdif by -\tbymin
  \multiply \tpanelheight by \tpdif
  \tpdif=\bymax \advance\tpdif by -\bymin
  \divide \tpanelheight by \tpdif
  \epsfig{file=#1,%
    bbllx=\bxmin bp,bblly=\tbymin bp,bburx=\bxmax bp,bbury=\bymax bp,%
    clip=,width=\panelwidth mm,height=\tpanelheight mm}}
\def\labelxypanel #1{%
  \ifnum\panelheight=0 
    \tpdif=\bymax \advance\tpdif by -\bymin
    \multiply \tpdif by \panelwidth
    \tpanelheight=\tpdif
    \tpdif=\bxmax \advance\tpdif by -\bxmin
    \divide \tpanelheight by \tpdif
  \else \tpanelheight=\panelheight \fi
  \tpdif=\bxmax \advance\tpdif by -\tbxmin
  \tpanelwidth=\panelwidth \multiply \tpanelwidth by \tpdif
  \tpdif=\bxmax \advance\tpdif by -\bxmin
  \divide \tpanelwidth by \tpdif 
  \tpdif=\bymax \advance\tpdif by -\tbymin 
  \multiply \tpanelheight by \tpdif
  \tpdif=\bymax \advance\tpdif by -\bymin
  \divide \tpanelheight by \tpdif
  \epsfig{file=#1,%
    bbllx=\tbxmin bp,bblly=\tbymin bp,bburx=\bxmax bp,bbury=\bymax bp,%
    clip=,width=\tpanelwidth mm,height=\tpanelheight mm}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% panel label
%% adds labels to panels, from Louis Strous
%% eg \panellabel{1.5em}{0.5em}{(a)} = 1.5em from right, 0.5em from bottom
\newcommand{\panellabel}[3]{\makebox[0pt][r]{\raisebox{#2} #3 \hspace{#1}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% float params
\def\topfraction{0.99}                      %% to permit many large figures
\def\dbltopfraction{0.99}
\def\textfraction{0.01} 
\def\floatpagefraction{0.99}
  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% COMMENTS
%% Option for yes/no printing of internal comments within LaTeX output.
%% - Begin comment with new line with %CC 
%% - start each comment line with %, for example with %RR
%% - end comment with new line with %EE and blank line if paragraph end.
%% - example:
%%      %CC
%%      %RR This is a RR comment to his co-authors
%%      %EE
%%
%% For comment printing replace with editor everywhere (after the
%% \begin{document} command):
%%        %CC by \CC 
%%        %EE by \end{verbatim} \EE          
%% and change these back again for skipping comments in LaTeX printout.
%% The other text will be compressed when comments are printed.
%%
%% Skip comments permanently by taking out CC and EE lines. 
%% Don't delete comments if you wish to record evolutionary thinking.  
%%
\def\CC{\par \vspace*{-2ex} \footnotesize \baselineskip=8pt \begin{verbatim}}
\def\EE{\par \vspace*{-2ex} \normalsize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% IGNORE
\long\def\startignore #1\stopignore{}   %% use \startignore....\stopignore

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% FULLFIGURE
%% for full-page figure with LaTeX caption use (Mats):
%%      \begin{figure}[p]
%%            \vbox to \textheight{\hbox{}\vfill
%%                  \caption[..]{\it............
%%                               \label{.....}}}
%%      \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% TASK
\newenvironment{task}{%
  \begin{list}{$\bullet$}{\itemsep=1ex \parindent=3ex \parskip=1ex 
    \topsep=0ex}}
  {\end{list}}        

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% CAMERA-READY ARTICLE HEADER
%% use for example: 
%%      \begin{koprr}
%%              {\large \bf  TITLE}\\[2ex]
%%              {\bf  AUTHORS}\\[2ex]
%%              {\sl  ADRRESS}\\[3cm]
%%      \end{koprr}
%%
\def\koprr{\list{}{      
  \itemindent=0pt \listparindent=0pt \itemsep=0pt
  \leftmargin=5ex}\item[]}                     %% 5ex = left margin
  \let\endkoprr=\endlist

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% FIGURETTE COLUMN
%% Blank column on the right for small figures.  Example: Seattle review
%% See also TeX parshape command and FLOATFIG style
%%
\def\kolom{\list{}{\rightmargin=5cm      %% 5cm = width column at right
  \topsep=0ex \itemsep=0cm \parsep=0ex \parskip=0ex \partopsep=0ex 
  \listparindent=3ex
  \itemindent=0pt \leftmargin=0pt} \item[] 
  \vspace*{-0ex}}                        %% this funny command kills gaps
  \let\endkolom=\endlist

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% LIST PARAMETERS
\renewcommand{\labelitemi}{{\bf --}}                %% no bullets but dashes
\def\setlistparams{         
  \topsep=0.7ex                 %% ADAPT: parskip=0: 0.7;  parskip=1: -1.2ex
  \itemsep=0.7ex                %% space between items
  \leftmargini=3ex}             %% dashes at beginning of line 
\setlistparams                  %% recall after type changes 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ALPHABETIC LIST
\newcounter{alistindex}  \newcounter{alistvalue}     %% problems: a)  b) etc
\newenvironment{alist}{%
   \begin{list}{\alph{alistindex})}{\usecounter{alistindex}}
   \itemsep=1.5ex \parskip=1ex}{\end{list}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% LINE SPACING
\def\spacing #1{\small \renewcommand{\baselinestretch}{#1}
                \normalsize \setlistparams}             %% eg: \spacing{1.5}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% UNINDENTED ITEMIZE
%% puts dashes fully left, no extra indent.  As ENUMERR below.
\newenvironment{itemrr}{\vspace*{-\parskip}
  \leftmargini=3ex \topsep=0.6ex       
  \begin{itemize}
     \itemsep=0.5ex \parindent=0ex \parsep=0ex}{
  \end{itemize} \vspace*{-\parskip}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% CONDENSED ITEMIZE
%% puts dashes fully left, no extra indent, small top and bottom spacing
%%                                   Example: Solar Physics Newsletter 3
\newenvironment{conditem}{               
  \leftmargini=6ex \topsep=0.2ex 
  \begin{itemize}
     \itemsep=0ex \parindent=3ex \parsep=0ex}{
  \end{itemize}}        

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% UNINDENTED ENUMERATE
%% puts numbers fully left, no extra indent.  Example: Kiev IAU Summary
\newenvironment{enumerr}{               
  \leftmargini=3ex \topsep=1.5ex       
  \begin{enumerate}
     \itemsep=0.7ex \parindent=3ex \parsep=0ex}{
  \end{enumerate}}        

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% CONDENSED ENUMERATE
%% puts numbers fully left, no extra indent, small top and bottom spacing.
%% Example: Solar Physics Newsletter 2 Huber item
\newenvironment{condenum}{               
  \leftmargini=3ex \topsep=0.5ex 
  \begin{enumerate}
     \itemsep=0ex \parindent=3ex \parsep=0ex}{
  \end{enumerate}}        

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ROMAN ENUMERATE
%% puts numbers fully left, uses (i), (ii), (iii) etc.                 
\newcounter{romenumnr}
\newenvironment{romanenum}{
  \leftmargini=5ex \topsep=1.5ex
  \begin{list}{(\roman{romenumnr}) --}{\usecounter{romenumnr}
      \itemsep=1ex \listparindent=3ex \parsep=0ex}}{
  \end{list}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% POSTER PAGE
%% one page, shadowframe, large sansserif, for POSTER.TPL
%% usage: \posterpage{header}{text}  
%%        suppress header with {\mbox{}}
%%        text may contain titles, multiple paragraphs, item lists etc.
\newcommand{\posterpage}[2]{{\Large \sf \newpage
  \setlength{\minipagewidth}{\textwidth} \addtolength{\minipagewidth}{-2cm}
  \fboxrule=0.3ex \fboxsep=0ex
  \def\shadowparams{\topsep=-2.5ex \itemsep=-1.5ex \leftmargini=5ex}
  \renewcommand{\labelitemi}{$\bullet$}
  \parskip=3ex \shadowparams
  \savebox{\boxcontent}[\textwidth]{
    \begin{minipage}[t]{\minipagewidth}
        \parskip=3ex \vspace*{1ex}
        \begin{center} \LARGE \bf #1 \end{center} 
        \vspace{2ex} #2 \vspace*{3ex} \mbox{ }
    \end{minipage}}
  \hspace*{\textwidth} \hspace*{-0.8ex} \rule{2ex}{\dp\boxcontent}
  \par \vspace*{-\dp\boxcontent} \vspace*{-7.2ex}
  \framebox[\textwidth]{\usebox{\boxcontent}}
  \par \vspace*{-3.0ex} \hspace*{1.7ex} \rule{\textwidth}{2ex}
  \setlistparams \renewcommand{\labelitemi}{{\bf --}}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% VWGRAPH
%% usage: \vwgraph{width}{header}{text}  
%%        suppress header with: \vwgraph{\mbox{}}{text} 
%%        specify fonts, eg: \vwgraph{\huge \bf ...}{\Large \sf ...}
%%        text may contain titles, paragraphs, item lists etc.
\newcommand{\vwgraph}[3]{\newpage
    \begin{center}
     \shadowframe{#1}{
       \begin{center}
         \vspace*{2ex}
         {\Large \bf #2}\\[4ex]
       \end{center}
       {\Large \sf #3}}   %% ADAPT font
     \end{center}}
\newenvironment{itemvg}{
  \leftmargini=3ex \topsep=0.5ex
  \begin{itemize} \vspace{-1ex}
     \itemsep=0.5ex \parindent=3ex \parsep=0ex}{
  \end{itemize}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% LECTVW
%% usage: \lectvw{header}{text}  = \vwgraph without shadow box
%%        suppress header with: \vwgraph{\mbox{}}{text} 
%%        specify fonts, eg: \vwgraph{\huge \bf ...}{\Large \sf ...}
%%        text may contain titles, paragraphs, item lists etc.
\long\def\lectvw#1#2{\newpage \vspace*{-15mm}
    \begin{center}
       \begin{center}
         {\LARGE \sc \underline{#1}}\\[4ex]
       \end{center}
       {\Large \sf #2}   %% ADAPT font
     \end{center}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SHADOWFRAME
%% minipage in shadowframe, used in VWGRAPH.TPL 
%% usage: \shadowframe{width}{text}
%%        eg: \shadowframe{15cm}{\large \sf ...}
%%        text may contain titles, paragraphs, item lists etc.
\newlength{\minipagewidth}
\newcommand{\shadowframe}[2]{
  \setlength{\minipagewidth}{#1} \addtolength{\minipagewidth}{-1cm}
  \fboxrule=0.5ex \fboxsep=0ex
  \def\shadowparams{\topsep=-2.5ex \itemsep=-1.5ex \leftmargini=5ex}
  \renewcommand{\labelitemi}{$\bullet$}
  \parskip=3ex \shadowparams 
  \savebox{\boxcontent}[#1]{         
    \begin{minipage}[t]{\minipagewidth}
      \vspace*{1.5ex} #2 \vspace*{0.5ex} \mbox{ } 
    \end{minipage}}
  \hspace*{#1} \hspace*{1.0ex} \rule{2ex}{\dp\boxcontent}  
  \par \vspace*{-\dp\boxcontent} \vspace*{-7.9ex} 
  \framebox[#1]{\usebox{\boxcontent}}  
  \par \vspace*{-3.0ex} \hspace*{4.5ex} \rule{#1}{2ex}
  \setlistparams \renewcommand{\labelitemi}{{\bf --}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% OVALHEAD
%% header in centered oval, 3 widths (8cm, 12cm, 16cm), for VWGRAPH.TPL
%% usage: \ovalhead{text}     eg: \ovalhead{\Large \bf Conclusions}
%%        \ovalhead{\mbox{}} suppresses oval
\newsavebox{\boxcontent}
\newcommand{\ovalhead}[1]{
  \unitlength=1cm
  \sbox{\boxcontent}{\mbox{~~{#1}~~}}
  \begin{center}
    \ifdim\wd\boxcontent>6ex 
    \ifdim\wd\boxcontent<8cm 
    \begin{picture}(8,3) \thicklines     
      \put(4.0,0.8){\oval(8,1.6)} 
      \put(0.0,0.7){\parbox{8cm}{
         \begin{center} \usebox{\boxcontent} \end{center}}}
    \end{picture}
    \else \ifdim\wd\boxcontent<12cm 
    \begin{picture}(12,3) \thicklines     
        \put(6.0,0.8){\oval(12,1.6)} 
        \put(0.0,0.7){\parbox{12cm}{
           \begin{center} \usebox{\boxcontent} \end{center}}}
    \end{picture}
    \else
    \begin{picture}(16,3) \thicklines     
        \put(8.0,0.8){\oval(16,1.6)} 
        \put(0.0,0.7){\parbox{16cm}{
           \begin{center} \usebox{\boxcontent} \end{center}}}
    \end{picture}
    \fi \fi \fi
  \end{center}} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% COLLOQFRAME
%% shadowed frame, for colloquium and lunch talk announcements
%% use: \colloqframe{width}{text}
\newcommand{\colloqframe}[2]{
  \setlength{\minipagewidth}{#1} \addtolength{\minipagewidth}{-1cm}
  \fboxrule=0.5ex \fboxsep=0ex
  \parskip=3ex
  \savebox{\boxcontent}[#1]{
    \begin{minipage}[t]{\minipagewidth}
      \vspace*{1.5ex} #2 \vspace*{0.5ex} \mbox{ }
    \end{minipage}}
  \hspace*{#1} \hspace*{-0.8ex} \rule{2ex}{\dp\boxcontent}
  \par \vspace*{-\dp\boxcontent} \vspace*{-7.9ex}
  \framebox[#1]{\usebox{\boxcontent}}
  \par \vspace*{-3.0ex} \hspace*{1.7ex} \rule{#1}{2ex}
  \renewcommand{\labelitemi}{{\bf --}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SOL OVAL
%% Old Utrecht sol symbol in label oval for SIU announcement labels 
%% Use: \soloval{text}
\newcommand{\soloval}[1]{\fboxrule=0.5mm \unitlength=1cm
\hspace*{5mm} \sol{20mm}\\[-20mm]
\begin{picture}(15,3) \thicklines
 \put(7.5,2){\oval(15.60,3.60)} \put(7.5,2){\oval(15.55,3.55)}
 \put(7.5,2){\oval(15.50,3.50)} \put(7.5,2){\oval(15.45,3.45)}
 \put(7.5,2){\oval(15.40,3.40)} \put(7.5,2){\oval(15.35,3.35)}
 \put(7.5,2){\oval(15.00,3.00)} \put(2.0,1.9){\parbox{13cm}{#1}}
\end{picture}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SECTION NUMBERING DEPTH
\setcounter{secnumdepth}{3}
\setcounter{tocdepth}{3}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SECTIONRR COMMANDS
                             %% use these for parskip>0 and/or to set labels
\def\chapterrr#1{\chapter{#1} \label{chap:#1} \vskip-\parskip}  
\def\sectionrr#1{\section{#1} \label{sec:#1} \vskip-\parskip}
\def\subsectionrr#1{\subsection{#1} \label{sec:#1} \vskip-\parskip}
\def\subsubsectionrr#1{\subsubsection{#1} \label{sec:#1}  \vskip-\parskip}
\def\paragraphrr#1{\paragraph{#1.} \label{sec:#1} \vskip-\parskip}
                                                     %% #1 without period

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SMALL SECTION HEAD 
\def\smallhead #1{\vspace{2ex} \noindent {\bf #1}~~~\noindent} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% CAMERA-READY SECTION HEADS
%% Alternative section heads for camera-ready output.
%% Use:    blank line + \head{SECTION HEADER} + blank line
%%         blank line + \subhead{Subsection Header} + blank line 
%%         blank line + \subsubhead{Subsubsection Header} + blank line
%% Note: often usage of e.g. \subsubsection*{3. Results} is better to
%%       obtain a smaller header since this won't occur at page bottom
\newcounter{headnr}            
\newcounter{subheadnr}[headnr]
\newcounter{subsubheadnr}[subheadnr]
\def\head #1\par{
  \stepcounter{headnr}                          %% sets subheadnr = 0 too 
  \vspace{2ex} \noindent                        %% 2ex = space above, no *
  {\bf \theheadnr~~~~#1}\\[1ex] \noindent}      %% 1ex = space below
\def\subhead #1\par{  
  \stepcounter{subheadnr}
  \vspace{1.3ex} \noindent
  {\bf \theheadnr.\arabic{subheadnr}~~~#1}\\[0.3ex] \noindent}
\def\subsubhead #1\par{
  \stepcounter{subsubheadnr}
  \vspace{1.0ex} \noindent
  {\bf \theheadnr.\arabic{subheadnr}.\arabic{subsubheadnr}~~~#1}\\ \noindent}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SPS-EPS NEWSLETTER MACROS 
\def\epstitle #1{\parskip=0ex \vspace{-2ex}
          \subsubsection*{\center \framebox[8.5cm]{\large \bf #1}}
          \parindent=3ex \parskip=0ex}
\def\epsdoubletitle #1#2{\parskip=0ex \vspace{-2ex}
          \subsubsection*{\center {\large \sc #1}}
          \vspace{-0.3ex}
          {\center \framebox[8.5cm]{\large \bf #2}\\[1ex]}
          \parindent=3ex \parskip=0ex \noindent}
\def\epssmalltitle #1{\subsubsection*{
        \vspace{-5ex} \center {\normalsize \sl #1}} \vspace*{-1.0ex}}
\def\epsauthor #1{\par\vspace*{0.3ex} \hspace*{\fill}{\sl#1}\\}
\def\epsinst #1{\hspace*{\fill}{\small#1}\\}
\def\sigrjr{\hspace{1.5cm} \raisebox{-1.5cm}{%
  \epsfig{file=/f4-usr1/rutten/adm/letters/figs/rjr.ps,%
     bbllx=75bp,bblly=300bp,bburx=480bp,bbury=500bp,clip=,%
     angle=-5,width=4cm}} \vspace*{-1.2cm} \par}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% DROPCAP
%%  big "miniature" from DROP.STY from Eric Bakker, use \dropcap{T}he
\font\dropfont= cmr12 scaled \magstep5
\def\dropcap#1#2{{\noindent
    \setbox0\hbox{\dropfont #1}\setbox1\hbox{#2}\setbox2\hbox{(}%
    \count0=\ht0\advance\count0 by\dp0\count1\baselineskip
    \advance\count0 by-\ht1\advance\count0by\ht2
    \dimen1=.5ex\advance\count0by\dimen1\divide\count0 by\count1
    \advance\count0 by1\dimen0\wd0
    \advance\dimen0 by.25em\dimen1=\ht0\advance\dimen1 by-\ht1
    \global\hangindent\dimen0\global\hangafter-\count0
    \hskip-\dimen0\setbox0\hbox to\dimen0{\raise-\dimen1\box0\hss}%
    \dp0=0in\ht0=0in\box0}#2}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% HANGLINE
%% next line indentation.  Usage: \hangline{2ex}.  End last with paragraph
\def\hangline #1{\parskip=0pt\par\noindent\hangafter=1\hangindent=#1}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% LATIN ABBREVIATIONS
\def\rmit#1{{\it #1}}              %% italics (RR style, Kluwer)
                                   %% redefine for A&A and ApJ, no italics
\def\etal{\rmit{et al.}}           %% use \etal\ for space behind it        
\def\etc{\rmit{etc.}}           
\def\ie{\rmit{i.e.,}}              %% , required (Webster 1681)
\def\eg{\rmit{e.g.,}}              %% , required (Webster 1681)
\def\cf{cf.}                       %% no Latin, always Roman (Webster 1686)
\def\viz{\rmit{viz.}}
\def\vs{\rmit{vs.}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SPECTRA
\def\specchar#1{\uppercase{#1}}    %% to be redefined for A&A, small caps
\def\AlI{\mbox{Al\,\specchar{i}}}  %% \def, not \newcommand, for overwrites 
\def\BI{\mbox{B\,\specchar{i}}}    %% use \AlI\ for space behind it
\def\BII{\mbox{B\,\specchar{ii}}}  
\def\BaI{\mbox{Ba\,\specchar{i}}}  
\def\BaII{\mbox{Ba\,\specchar{ii}}} 
\def\CI{\mbox{C\,\specchar{i}}} 
\def\CII{\mbox{C\,\specchar{ii}}} 
\def\CIII{\mbox{C\,\specchar{iii}}} 
\def\CIV{\mbox{C\,\specchar{iv}}} 
\def\CaI{\mbox{Ca\,\specchar{i}}} 
\def\CaII{\mbox{Ca\,\specchar{ii}}} 
\def\CaIII{\mbox{Ca\,\specchar{iii}}} 
\def\CoI{\mbox{Co\,\specchar{i}}} 
\def\CrI{\mbox{Cr\,\specchar{i}}} 
\def\CrII{\mbox{Cr\,\specchar{ii}}} 
\def\CsI{\mbox{Cs\,\specchar{i}}} 
\def\CsII{\mbox{Cs\,\specchar{ii}}} 
\def\CuI{\mbox{Cu\,\specchar{i}}} 
\def\FeI{\mbox{Fe\,\specchar{i}}} 
\def\FeII{\mbox{Fe\,\specchar{ii}}} 
\def\FeXVI{\mbox{Fe\,\specchar{xvi}}}
\def\FrI{\mbox{Fr\,\specchar{i}}}
\def\HI{\mbox{H\,\specchar{i}}} 
\def\HII{\mbox{H\,\specchar{ii}}} 
\def\Hmin{\hbox{\rmH$^{^{_-}}\!$}}      %% H^min, very elegant
\def\Hemin{\hbox{{\rm He}$^{^{_-}}$}}    %% He^min, idem
\def\HeI{\mbox{He\,\specchar{i}}} 
\def\HeII{\mbox{He\,\specchar{ii}}} 
\def\HeIII{\mbox{He\,\specchar{iii}}} 
\def\KI{\mbox{K\,\specchar{i}}} 
\def\KII{\mbox{K\,\specchar{ii}}} 
\def\KIII{\mbox{K\,\specchar{iii}}} 
\def\LiI{\mbox{Li\,\specchar{i}}} 
\def\LiII{\mbox{Li\,\specchar{ii}}} 
\def\LiIII{\mbox{Li\,\specchar{iii}}} 
\def\MgI{\mbox{Mg\,\specchar{i}}} 
\def\MgII{\mbox{Mg\,\specchar{ii}}} 
\def\MgIII{\mbox{Mg\,\specchar{iii}}} 
\def\MnI{\mbox{Mn\,\specchar{i}}} 
\def\NI{\mbox{N\,\specchar{i}}}
\def\NaI{\mbox{Na\,\specchar{i}}}
\def\NaII{\mbox{Na\,\specchar{ii}}}
\def\NaIII{\mbox{Na\,\specchar{iii}}} 
\def\NiI{\mbox{Ni\,\specchar{i}}} 
\def\NiII{\mbox{Ni\,\specchar{ii}}}
\def\NiIII{\mbox{Ni\,\specchar{iii}}} 
\def\OI{\mbox{O\,\specchar{i}}} 
\def\OVI{\mbox{O\,\specchar{vi}}}
\def\RbI{\mbox{Rb\,\specchar{i}}} 
\def\RrI{\mbox{Rr\,\specchar{i}}}      %% Robruttenium I
\def\RrII{\mbox{Rr\,\specchar{ii}}}    %% Robruttenium II
\def\RrIII{\mbox{Rr\,\specchar{iii}}}  %% Robruttenium III
\def\SII{\mbox{S\,\specchar{ii}}} 
\def\SiI{\mbox{Si\,\specchar{i}}} 
\def\SiII{\mbox{Si\,\specchar{ii}}} 
\def\SrI{\mbox{Sr\,\specchar{i}}}
\def\SrII{\mbox{Sr\,\specchar{ii}}}
\def\TiI{\mbox{Ti\,\specchar{i}}} 
\def\TiII{\mbox{Ti\,\specchar{ii}}} 
\def\TiIII{\mbox{Ti\,\specchar{iii}}} 
\def\TiIV{\mbox{Ti\,\specchar{iv}}} 
\def\VI{\mbox{V\,\specchar{i}}} 
\def\HtwoO{\mbox{H$_2$O}}        %% H2O
\def\Otwo{\mbox{O$_2$}}          %% O2

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% LINES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% hydrogen
\def\Halpha{\mbox{H$\alpha$}}           %% use \Halpha\ for space behind it
\def\Ha{\mbox{H$\alpha$}}
\def\Hbeta{\mbox{H$\beta$}}
\def\Hepsilon{\mbox{H$\epsilon$}}
\def\Bacont{\mbox{Ba\,{\small cont}}}
\def\Lyalpha{\mbox{Ly$\,\alpha$}}
\def\Lybeta{\mbox{Ly$\,\beta$}}
\def\Lycont{\mbox{Ly\,{\small cont}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Na D
\def\NaD{\mbox{Na\,\specchar{i}\,D}}    %% use \NaD\ for space behind it
\def\NaDone{\mbox{Na\,\specchar{i}\,\,D$_1$}}
\def\NaDtwo{\mbox{Na\,\specchar{i}\,\,D$_2$}}
\def\NaID{\mbox{Na\,\specchar{i}\,\,D}}
\def\NaIDone{\mbox{Na\,\specchar{i}\,\,D$_1$}}
\def\NaIDtwo{\mbox{Na\,\specchar{i}\,\,D$_2$}}
\def\Done{\mbox{D$_1$}}
\def\Dtwo{\mbox{D$_2$}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Mg b
\def\Mgbone{\mbox{Mg\,\specchar{i}\,b$_1$}}
\def\Mgbtwo{\mbox{Mg\,\specchar{i}\,b$_2$}}
\def\Mgbthree{\mbox{Mg\,\specchar{i}\,b$_3$}}
\def\MgIb{\mbox{Mg\,\specchar{i}\,b}}
\def\MgIbone{\mbox{Mg\,\specchar{i}\,b$_1$}}
\def\MgIbtwo{\mbox{Mg\,\specchar{i}\,b$_2$}}
\def\MgIbthree{\mbox{Mg\,\specchar{i}\,b$_3$}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Ca II H & K 
\def\CaIIK{\mbox{Ca\,\specchar{ii}\,\,K}}       %% use \CaIIK\ for space
\def\CaIIH{\mbox{Ca\,\specchar{ii}\,\,H}}
\def\CaIIHK{\mbox{Ca\,\specchar{ii}\,\,H\,\&\,K}}
\def\HK{\mbox{H\,\&\,K}}
\def\Kthree{\mbox{K$_3$}}      %% numbers not permitted, dammit
\def\Hthree{\mbox{H$_3$}}
\def\Ktwo{\mbox{K$_2$}}
\def\Htwo{\mbox{H$_2$}}
\def\Kone{\mbox{K$_1$}}     
\def\Hone{\mbox{H$_1$}}     
\def\KtwoV{\mbox{K$_{2V}$}}
\def\KtwoR{\mbox{K$_{2R}$}}
\def\KoneV{\mbox{K$_{1V}$}}
\def\KoneR{\mbox{K$_{1R}$}}
\def\HtwoV{\mbox{H$_{2V}$}}
\def\HtwoR{\mbox{H$_{2R}$}}
\def\HoneV{\mbox{H$_{1V}$}}
\def\HoneR{\mbox{H$_{1R}$}}
\def\Kg{{\KtwoV\ grain}}
\def\Kgs{{\KtwoV\ grains}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Mg II h & k 
\def\hk{\mbox{h\,\&\,k}}
\def\kthree{\mbox{k$_3$}}    
\def\hthree{\mbox{h$_3$}}
\def\ktwo{\mbox{k$_2$}}
\def\htwo{\mbox{h$_2$}}
\def\kone{\mbox{k$_1$}}     
\def\hone{\mbox{h$_1$}}     
\def\ktwoV{\mbox{k$_{2V}$}}
\def\ktwoR{\mbox{k$_{2R}$}}
\def\koneV{\mbox{k$_{1V}$}}
\def\koneR{\mbox{k$_{1R}$}}
\def\htwoV{\mbox{h$_{2V}$}}
\def\htwoR{\mbox{h$_{2R}$}}
\def\honeV{\mbox{h$_{1V}$}}
\def\honeR{\mbox{h$_{1R}$}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ATOMIC LEVEL
%% use:    \level 3s3p 3Pe
%%         \level 3s$^2$ {1,3}P{e,o}
%%         \level {} 3Ge
%%
\def\level #1 #2#3#4{$#1 \: ^{#2} \mbox{#3} ^{#4}$}   

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% STAR NAME
\newcommand{\starname}[2]{${#1}$\,{\rm {#2}}}  %% \starname{\alpha}{Cen~A} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ROMAN CHARACTERS FOR MATH 
\def\rma{{\rm a}} \def\rmA{{\rm A}}             %% without space 
\def\rmb{{\rm b}} \def\rmB{{\rm B}}             %% use for indices etc. 
\def\rmc{{\rm c}} \def\rmC{{\rm C}} 
\def\rmd{{\rm d}} \def\rmD{{\rm D}} 
\def\rme{{\rm e}} \def\rmE{{\rm E}} 
\def\rmf{{\rm f}} \def\rmF{{\rm F}} 
\def\rmg{{\rm g}} \def\rmG{{\rm G}} 
\def\rmh{{\rm h}} \def\rmH{{\rm H}} 
\def\rmi{{\rm i}} \def\rmI{{\rm I}} 
\def\rmj{{\rm j}} \def\rmJ{{\rm J}} 
\def\rmk{{\rm k}} \def\rmK{{\rm K}} 
\def\rml{{\rm l}} \def\rmL{{\rm L}} 
\def\rmm{{\rm m}} \def\rmM{{\rm M}} 
\def\rmn{{\rm n}} \def\rmN{{\rm N}} 
\def\rmo{{\rm o}} \def\rmO{{\rm O}} 
\def\rmp{{\rm p}} \def\rmP{{\rm P}} 
\def\rmq{{\rm q}} \def\rmQ{{\rm Q}} 
\def\rmr{{\rm r}} \def\rmR{{\rm R}} 
\def\rms{{\rm s}} \def\rmS{{\rm S}} 
\def\rmt{{\rm t}} \def\rmT{{\rm T}} 
\def\rmu{{\rm u}} \def\rmU{{\rm U}} 
\def\rmv{{\rm v}} \def\rmV{{\rm V}} 
\def\rmw{{\rm w}} \def\rmW{{\rm W}} 
\def\rmx{{\rm x}} \def\rmX{{\rm X}} 
\def\rmy{{\rm y}} \def\rmY{{\rm Y}} 
\def\rmz{{\rm z}} \def\rmZ{{\rm Z}} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% UNITS
\def\deg{\hbox{$^\circ$}}       %% \def for overwriting, \box for math
\def\degree{\hbox{$^\circ$}}
\def\degrees{\hbox{$^\circ$}}
\def\arcmin{\hbox{$^\prime$}}
\def\bgmin{\hbox{$^\prime$}}
\def\arcsec{\hbox{$^{\prime\prime}$}}
\def\secarc{\hbox{$^{\prime\prime}$}}
\def\bgsec{\hbox{$^{\prime\prime}$}}
\def\kms{\hbox{km$\;$s$^{-1}$}}
\def\micron{\hbox{$\mu$m}}
\def\kayser{\hbox{$\rm cm^{-1}$}}
\def\Mxcm{\hbox{Mx\,cm$^{-2}$}}    %% no 2, damn tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% VARIA
\def\dif{\: {\rm d}}                       %% differential d with space
\def\ep{\:{\rm e}^}                        %% e^ with space and roman e
\def\lambdop{\hbox{$\bf \Lambda$}}         %% plain Lambda operator

\def\gf{\mbox{$g \! f$}}                   %% \gf\ for space behind it

\def\ko{($k, \omega$)}                     %% k - omega 
\def\komega{($k, \omega$)}                 %% k - omega 
\def\VminI{\hbox{$V\!\!-\!\!I$}}           %% V-I
\def\IminI{\hbox{$I\!\!-\!\!I$}}           %% I-I
\def\VminV{\hbox{$V\!\!-\!\!V$}}           %% V-V
\def\Xt{\hbox{$X\!\!-\!t$}}                %% X-t

\def\sun{\hbox{$\odot$}}                   %% Sun symbol
\def\earth{\hbox{$\oplus$}}                %% Earth symbol

\def\BminV{\hbox{$B\!\!-\!\!V$}}           %% B-V
\def\VminIk{\hbox{$(V\!\!-\!\!I)_K$}}      %% V-I_K
\def\Teff{\hbox{$T_{\rm eff}$}}            %% T_eff

\def\Bapp{\hbox{$B_{\rm app}$}}              %% apparent flux density
\def\Basp{\hbox{$B_{\rm app}^{\rm ASP}$}}    %% apparent flux density ASP
\def\Bbbso{\hbox{$B_{\rm app}^{\rm BBSO}$}}  %% idem BBSO
\def\Bkpno{\hbox{$B_{\rm app}^{\rm KPNO}$}}  %% idem KPNO

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% stacked math symbols
%% macro by Louis Strous, after char.mac Skumanich Soesterberg 
%% usage: \mathstacksym\newsymbol{upper_symbol}{lower_symbol}
%%                               {upper_height}{lower_depth}
\def\mathstacksym#1#2#3#4#5{\def#1{\mathrel{\hbox to 0pt{\lower 
    #5\hbox{#3}\hss} \raise #4\hbox{#2}}}}

\mathstacksym\lta{$<$}{$\sim$}{1.5pt}{3.5pt} % less than approximately
\mathstacksym\gta{$>$}{$\sim$}{1.5pt}{3.5pt} % greater than approximately
\mathstacksym\lrarrow{$\leftarrow$}{$\rightarrow$}{2pt}{1pt} % equilibrium
\mathstacksym\lessgreat{$>$}{$<$}{3pt}{3pt} %% less or greater

%%%%%%%%%%%%%%%%%%%%  END OF FILE RRMACROS.TEX  %%%%%%%%%%%%%%%%%%%%%%%%%%%


==> h3319aa <==
%% file: AAJOUR.BIB = journal strings, new AA & AoJ abbreviations
%% last: Oct 31 1995
%% baton: Rob Rutten, Sterrekundig Instituut Utrecht
%%     >> don't change this file - its baton is mine all the time <<

@STRING{acta = "Acta Astron."}
@STRING{actastsin = "Acta Astron.\ Sin."}
@STRING{actapsin = "Acta Astrophys.\ Sin."}
@STRING{advp = "Adv.\ Phys."}
@STRING{advsr = "Adv.\ Space Res."}
@STRING{amjp = "Am.\ J.\ Phys."}
@STRING{annap = "Ann.\ d'Astrophys."}
@STRING{annrev = "ARA\hbox{\rm \&}A"}
@STRING{araa = "ARA\hbox{\rm \&}A"}
@STRING{ao = "Appl.\ Opt."}
@STRING{appl = "Appl.\ Phys.\ Lett."}
@STRING{apb = "Appl.\ Phys.\ B"}
@STRING{afz = "Afz"}
@STRING{aa = "A\hbox{\rm \&}A"}
@STRING{aar = "A\hbox{\rm \&}AR"}
@STRING{aas = "A\hbox{\rm \&}AS"}
@STRING{agas = "Astron.\ Ges.\ Abstr.\ Ser."}
@STRING{aj = "AJ"}
@STRING{an = "Astron.\ Nachr."}
@STRING{azh = "AZh"}
@STRING{apj = "ApJ"}
@STRING{apjl = "ApJ"}
@STRING{apjss = "ApJS"}
@STRING{apss = "Ap\hbox{\rm \&}SS"}
@STRING{ap = "Astrophysics"}
@STRING{ajp = "Aust.\ J.\ Phys."}
@STRING{baas = "BAAS"}
@STRING{ban = "Bull.\ Astron.\ Inst.\ Neth."}
@STRING{bac = "Bull.\ Astron.\ Inst.\ Czech."}
@STRING{cjp = "Can.\ J.\ Phys."}
@STRING{cm = "Celest.\ Mech."}
@STRING{chinaa = "Chin.\ Astron."}
@STRING{cast = "Comments Astrophys."}
@STRING{fiz = "Fizika"}
@STRING{gafd = "Geophys.\ Astrophys.\ Fluid Dyn."}
@STRING{gj = "Geophys.\ J."}
@STRING{grl = "Geophys.\ Res.\ Lett."}
@STRING{geo = "Geophysics"}
@STRING{hd = "Hemel en Dampkring"}
@STRING{iauc = "IAU Circ."}
@STRING{iauib = "IAU Inf.\ Bull."}
@STRING{icarus = "Icarus"}
@STRING{jap = "J.\ Appl.\ Phys."}
@STRING{jaa = "JA\hbox{\rm \&}A"}
@STRING{jas = "J.\ Atmos.\ Sci."}
@STRING{jchemp = "J.\ Chem.\ Phys."}
@STRING{jcomp = "J.\ Comp.\ Phys."}
@STRING{jfm = "J.\ Fluid Mech."}
@STRING{jgr = "J.\ Geophys.\ Res."}
@STRING{jhast = "J.\ Hist.\ Astron."}
@STRING{jmolspec = "J.\ Mol.\ Spectrosc."}
@STRING{josa = "J.\ Opt.\ Soc.\ Am."}
@STRING{josaa = "J.\ Opt.\ Soc.\ Am.\ A"}
@STRING{josab = "J.\ Opt.\ Soc.\ Am.\ B"}
@STRING{jp = "J.\ Phys."}
@STRING{jpa = "J.\ Phys.\ A"}
@STRING{jpb = "J.\ Phys.\ B"}
@STRING{jpd = "J.\ Phys.\ D"}
@STRING{jpe = "J.\ Phys.\ E"}
@STRING{jpg = "J.\ Phys.\ G"}
@STRING{jpsj = "J.\ Phys.\ Soc.\ Japan"}
@STRING{jpp = "J.\ Plasma Phys."}
@STRING{jqsrt = "J.\ Quant.\ Spectrosc.\ Radiat.\ Transfer"}
@STRING{jrasc = "J.\ R.\ Astron.\ Soc.\ Can."}
@STRING{jetpl = "JETP Lett."}
@STRING{kfnt = "Kinematika Fiz.\ Nebesn.\ Tel"}
@STRING{msai = "Mem.\ Soc.\ Astron.\ Ital."}
@STRING{merc = "Mercury"}
@STRING{mag = "Mitt.\ Astron.\ Ges."}
@STRING{mn = "MNRAS"}
@STRING{mnras = "MNRAS"}
@STRING{mnassa = "Mon.\ Notes Astron.\ Soc.\ S.\ Afr."}
@STRING{nat = "Nat"}
@STRING{nature="Nat"}
@STRING{natwis = "Naturwissenschaften"}
@STRING{nattech = "Natuur en Techniek"}
@STRING{obs = "Observatory"}
@STRING{pfa = "Phys.\ Fluids A"}
@STRING{pfb = "Phys.\ Fluids B"}
@STRING{pla = "Phys.\ Lett.\ A"}
@STRING{plb = "Phys.\ Lett.\ B"}
@STRING{pra = "Phys.\ Rev.\ A"}
@STRING{prb = "Phys.\ Rev.\ B"}
@STRING{prc = "Phys.\ Rev.\ C"}
@STRING{prd = "Phys.\ Rev.\ D"}
@STRING{prl = "Phys.\ Rev.\ Lett."}
@STRING{ps = "Phys.\ Scr."}
@STRING{ptod = "Phys.\ Today"}
@STRING{pha = "Physica A"}
@STRING{phb = "Physica B"}
@STRING{phd = "Physica D"}
@STRING{pss = "Planet.\ Space Sci."}
@STRING{ppcf = "Plasma Phys.\ Controlled Fusion"}
@STRING{pasa = "Proc.\ Astron.\ Soc.\ Aust."}
@STRING{pi3e = "Proc.\ IEEE"}
@STRING{prsl = "Proc.\ R.\ Soc.\ London Ser.\ A"}
@STRING{posp = "Proceedings of SPIE"}
@STRING{pasj = "PASJ"}
@STRING{pasp = "PASP"}
@STRING{paspc = "PASPC"}
@STRING{qjras = "QJRAS"}
@STRING{ra = "Rev.\ Astron."}
@STRING{sciam = "Sci.\ Am."}
@STRING{sc = "Sci"}
@STRING{sky = "Sky Telesc."}
@STRING{sp = "Solar Phys."}
@STRING{sdb = "Soln.\ Dannye Byull."}
@STRING{sonne = "Sonne"}
@STRING{sa = "SvA"}
@STRING{sal = "SvA"}
@STRING{ssr = "Space Sci.\ Rev."}
@STRING{sf = "Spaceflight"}
@STRING{sterne = "Sterne"}
@STRING{sw = "Sterne Weltraum"}
@STRING{uao = "Upps.\ Astron.\ Obs.\ Rep."}
@STRING{va = "Vistas Astron."}
@STRING{zpa = "Z.\ Phys.\ A"}
@STRING{zpc = "Z.\ Phys.\ C"}
@STRING{zenit = "Zenit"}
@STRING{zetf = "Zh.\ Ehksp.\ Teor.\ Fiz."}
@STRING{ZsAp = "Zs.\ f.\ Ap."}
@STRING{ZsP = "Zs.\ f.\ Phys."}


==> h3319bib <==
@ARTICLE{Abia1988A&A...206..100A,
    author = {{Abia}, C. and {Rebolo}, R. and {Beckman}, J.\ E. and {Crivellari}, L.
        },
    title = {Abundances of light metals and NI in a sample of disc stars},
    journal = {\aap},
    year = 1988,
    month = nov,
    volume = 206,
    pages = {100--107},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1988A%26A...206..100A&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Abia1998MNRAS.293...89A,
    author = {{Abia}, C. and {Wallerstein}, G.},
    title = "Heavy-element abundances in seven SC stars and several related stars",
    journal = {\mnras},
    year = 1998,
    month = jan,
    volume = 293,
    pages = {89},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1998MNRAS.293...89A&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Achmad1991A&A...249..192A,
    author = {{Achmad}, L. and {de Jager}, C. and {Nieuwenhuijzen}, H.},
    title = {Atmospheric model parameters and shock wave field for the supergiant Alpha Carinae (F0Ib)},
    journal = {\aap},
    year = 1991,
    month = sep,
    volume = 249,
    pages = {192--198},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1991A%26A...249..192A&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Adelman1990ApJ...348..712A,
    author = {{Adelman}, S.\ J. and {Gulliver}, A.\ F.},
    title = "An elemental abundance analysis of the superficially normal A star VEGA",
    journal = {\apj},
    year = 1990,
    month = jan,
    volume = 348,
    pages = {712--717},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1990ApJ...348..712A&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Allard1992RMxAA..23..203A,
    author = {{Allard}, F. and {Scholz}, M. and {Wehrse}, R.},
    title = "Molecular opacities in M-star atmospheres.",
    journal = {Revista Mexicana de Astronomia y Astrofisica},
    year = 1992,
    month = mar,
    volume = 23,
    pages = {203--215},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1992RMxAA..23..203A&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Altas1987Ap&SS.134...85A,
    author = {{Altas}, L.},
    title = "Carbon, nitrogen, and oxygen abundances in Procyon, sun, and Arcturus",
    journal = {\apss},
    year = 1987,
    month = jun,
    volume = 134,
    pages = {85--94},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1987Ap%26SS.134...85A&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Anders1989GeCoA..53..197A,
    author = {{Anders}, E. and {Grevesse}, N.},
    title = "{Abundances of the elements - Meteoritic and solar}",
    journal = {\gca},
    year = 1989,
    month = jan,
    volume = 53,
    pages = {197--214},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1989GeCoA..53..197A&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{Aoki1997A&A...328..175A,
    author = {{Aoki}, W. and {Tsuji}, T.},
    title = "High resolution infrared spectroscopy of CN and NH lines:  nitrogen abundance in oxygen-rich giants through K to late M",
    journal = {\aap},
    year = 1997,
    month = dec,
    volume = 328,
    pages = {175--186},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1997A%26A...328..175A&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Aringer1999A&A...342..799A,
    author = {{Aringer}, B. and {H{\"o}fner}, S. and {Wiedemann}, G. and {Hron}, J. and 
        {J{\o}rgensen}, U.\ G. and {K{\"a}ufl}, H.\ U. and {Windsteig}, W.
        },
    title = "SiO rotation-vibration bands in cool giants II. The behaviour of SiO bands in AGB stars",
    journal = {\aap},
    year = 1999,
    month = feb,
    volume = 342,
    pages = {799--808},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1999A%26A...342..799A&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Asplund2000A&A...359..729A,
    author = {{Asplund}, M. and {Nordlund}, {\AA}. and {Trampedach}, R. and 
        {Allende Prieto}, C. and {Stein}, R.\ F.},
    title = {Line formation in solar granulation. I. Fe line shapes, shifts and asymmetries},
    journal = {\aap},
    year = 2000,
    month = jul,
    volume = 359,
    pages = {729--742},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2000A%26A...359..729A&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Ayres1982ApJ...263..791A,
    author = {{Ayres}, T.~R. and {Simon}, T. and {Linsky}, J.~L.},
    title = "{Evolution of chromospheres and coronae in solar mass stars - A far-ultraviolet and soft X-ray comparison of Arcturus /K2 III/ and Alpha Centauri A /G2 V/}",
    journal = {\apj},
    year = 1982,
    month = dec,
    volume = 263,
    pages = {791--802},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1982ApJ...263..791A&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Balona1984MNRAS.211..973B,
    author = {{Balona}, L.\ A.},
    title = "Calibration of effective temperature, bolometric correction and mass for early-type stars using Stroemgren photometric indices",
    journal = {\mnras},
    year = 1984,
    month = dec,
    volume = 211,
    pages = {973--979},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1984MNRAS.211..973B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Barklem2000A&A...355L...5B,
    author = {{Barklem}, P.\ S. and {Piskunov}, N. and {O'Mara}, B.\ J.},
    title = {Self broadening of hydrogen lines: initial results},
    journal = {\aap},
    year = 2000,
    month = mar,
    volume = 355,
    pages = {L5--L8},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2000A%26A...355L...5B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Barnes1976MNRAS.174..489B,
    author = {{Barnes}, T.\ G. and {Evans}, D.\ S.},
    title = "Stellar angular diameters and visual surface brightness. I. Late spectral types.",
    journal = {\mnras},
    year = 1976,
    month = mar,
    volume = 174,
    pages = {489--502},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1976MNRAS.174..489B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Barnes1976MNRAS.174..503B,
    author = {{Barnes}, T.\ G. and {Evans}, D.\ S. and {Parsons}, S.\ B.},
    title = "Stellar angular diameters and visual surface brightness. II. Early and intermediate spectral types.",
    journal = {\mnras},
    year = 1976,
    month = mar,
    volume = 174,
    pages = {503--512},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1976MNRAS.174..503B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Basri1979ApJ...234.1023B,
    author = {{Basri}, G.\ S. and {Linsky}, J.\ L.},
    title = "Outer atmospheres of cool stars. II - MG II flux profiles and chromospheric radiative loss rates",
    journal = {\apj},
    year = 1979,
    month = dec,
    volume = 234,
    pages = {1023--1035},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1979ApJ...234.1023B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Becker1981ApJS...45..475B,
    author = {{Becker}, S.~A.},
    title = "{The evolution of intermediate-mass stars from the zero-age main sequence to the base of the asymptotic giant branch as a function of mass and composition}",
    journal = {\apjs},
    year = 1981,
    month = mar,
    volume = 45,
    pages = {475--505},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1981ApJS...45..475B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Bell1981ApJ...248.1031B,
    author = {{Bell}, R.\ A. and {Dreiling}, L.\ A.},
    title = "The chemical composition, gravity, and temperature of Sirius",
    journal = {\apj},
    year = 1981,
    month = sep,
    volume = 248,
    pages = {1031--1042},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1981ApJ...248.1031B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Bell1985MNRAS.212..497B,
    author = {{Bell}, R.\ A. and {Edvardsson}, B. and {Gustafsson}, B.},
    title = "The surface gravity of Arcturus from MgH lines, strong metal lines and the ionization equilibrium of iron",
    journal = {\mnras},
    year = 1985,
    month = feb,
    volume = 212,
    pages = {497--515},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1985MNRAS.212..497B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Bell1989MNRAS.236..653B,
    author = {{Bell}, R.\ A. and {Gustafsson}, B.},
    title = "The effective temperatures and colours of G and K stars",
    journal = {\mnras},
    year = 1989,
    month = feb,
    volume = 236,
    pages = {653--707},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1989MNRAS.236..653B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Bessell1984PASP...96..247B,
    author = {{Bessell}, M.~S. and {Wood}, P.~R.},
    title = "{A note on bolometric corrections for late-type stars and long-period variables}",
    journal = {\pasp},
    year = 1984,
    month = mar,
    volume = 96,
    pages = {247--249},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1984PASP...96..247B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Bessell1998A&A...333..231B,
    author = {{Bessell}, M.~S. and {Castelli}, F. and {Plez}, B.},
    title = "{Model atmospheres broad-band colors, bolometric corrections  and temperature calibrations for O - M stars}",
    journal = {\aap},
    year = 1998,
    month = may,
    volume = 333,
    pages = {231--250},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1998A%26A...333..231B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Blackwell1977MNRAS.180..177B,
    author = {{Blackwell}, D.\ E. and {Shallis}, M.\ J.},
    title = {Stellar angular diameters from infrared photometry - Application to Arcturus and other stars; with effective temperatures},
    journal = {\mnras},
    year = 1977,
    month = jul,
    volume = 180,
    pages = {177--191},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1977MNRAS.180..177B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Blackwell1980A&A....82..249B,
    author = {{Blackwell}, D.\ E. and {Petford}, A.\ D. and {Shallis}, M.\ J.
        },
    title = {Use of the infra-red flux method for determining stellar effective temperatures and angular diameters - The stellar temperature scale},
    journal = {\aap},
    year = 1980,
    month = feb,
    volume = 82,
    pages = {249--252},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1980A%26A....82..249B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Blackwell1990A&A...232..396B,
    author = {{Blackwell}, D.\ E. and {Petford}, A.\ D. and {Haddock}, D.\ J. and 
        {Arribas}, S. and {Selby}, M.\ J.},
    title = {Determination of temperatures and angular diameters of 114 F-M stars using the infrared flux method (IRFM)},
    journal = {\aap},
    year = 1990,
    month = jun,
    volume = 232,
    pages = {396--410},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1990A%26A...232..396B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}
@ARTICLE{Blackwell1991A&A...245..567B,
    author = {{Blackwell}, D.\ E. and {Lynas-Gray}, A.\ E. and {Petford}, A.\ D.
        },
    title = "Effect of improved H$^-$ opacity on the infrared flux method temperature scale and derived angular diameters - Use of a self-consistent calibration", 
    journal = {\aap},
    year = 1991,
    month = may,
    volume = 245,
    pages = {567--574},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1991A%26A...245..567B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Blackwell1998A&AS..129..505B,
    author = {{Blackwell}, D.\ E. and {Lynas-Gray}, A.\ E.},
    title = "Determination of the temperatures of selected ISO flux calibration stars using the Infrared Flux Method",
    journal = {\aaps},
    year = 1998,
    month = may,
    volume = 129,
    pages = {505--515},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1998A%26AS..129..505B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{BohmVitense1981ARA&A..19..295B,
    author = {{B\"{o}hm-Vitense}, E.},
    title = "{The effective temperature scale}",
    journal = {\araa},
    year = 1981,
    volume = 19,
    pages = {295--317},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1981ARA%26A..19..295B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}



@ARTICLE{Bonnell1982MNRAS.201..253B,
    author = {{Bonnell}, J. and {Bell}, R.\ A.},
    title = "Carbon and nitrogen abundances in Population I G and K giant stars from DDO photometry",
    journal = {\mnras},
    year = 1982,
    month = oct,
    volume = 201,
    pages = {253--263},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1982MNRAS.201..253B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Bonnell1993MNRAS.264..319B,
    author = {{Bonnell}, J.~T. and {Bell}, R.~A.},
    title = "{The Gravities of K Giant Stars Determined from OI and OH Features}",
    journal = {\mnras},
    year = 1993,
    month = sep,
    volume = 264,
    pages = {319},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1993MNRAS.264..319B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Boyarchuk1983Ap.....18..228B,
    author = {{Boyarchuk}, A.\ A. and {Lyubimkov}, L.\ S.},
    title = {The Atmosphere of Canopus - Part One - Model of the Atmosphere and Distribution of the Microturbulence},
    journal = {Astrophysics},
    year = 1983,
    volume = 18,
    pages = {228},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1983Ap.....18..228B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Brown1974MNRAS.167..121B,
    author = {{Brown}, R.\ H. and {Davis}, J. and {Allen}, L.\ R.},
    title = {The angular diameters of 32 stars.},
    journal = {\mnras},
    year = 1974,
    month = apr,
    volume = 167,
    pages = {121--136},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1974MNRAS.167..121B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Brown1983ApJ...265L..93B,
    author = {{Brown}, J.\ A. and {Tomkin}, J. and {Lambert}, D.\ L.},
    title = {Evidence of non-LTE in photospheric lines of G and K giants},
    journal = {\apjl},
    year = 1983,
    month = feb,
    volume = 265,
    pages = {L93--L97},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1983ApJ...265L..93B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Brown1989ApJS...71..293B,
    author = {{Brown}, J.\ A. and {Sneden}, C. and {Lambert}, D.\ L. and {Dutchover}, E.\ J.
        },
    title = "A search for lithium-rich giant stars",
    journal = {\apjs},
    year = 1989,
    month = oct,
    volume = 71,
    pages = {293--322},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1989ApJS...71..293B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Burnashev1983IzKry..67...13B,
    author = {{Burnashev}, V.\ I.},
    title = "A determination of the effective temperatures, accelerations of gravity, and metallicity parameters of late-type stars from data on energy distribution in their spectra",
    journal = {Izvestiya Ordena Trudovogo Krasnogo Znameni Krymskoj Astrofizicheskoj Observatorii},
    year = 1983,
    volume = 67,
    pages = {13--33},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1983IzKry..67...13B&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}



@INPROCEEDINGS{Cami1997fiso.work..159C,                                       
        AUTHOR  = {{Cami}, J. and {Justtanont}, K. and {de Jong}, T. and {Feuchtgruber}, H. and 
        {Tielens}, A.\ G.\ G.\ M. and {Yamamura}, I. and {Waters}, L.\ B.\ F.\ M.
        }, 
        TITLE   = "CO$_2$ Emission in O-Rich AGB Stars",
        BOOKTITLE = {The first ISO workshop on Analytical Spectroscopy},
        YEAR    = 1997,
        PAGES   = {159},
      EDITOR    = {{Heras}, A.\ M. and {Leech}, K. and {Trams}, N.\ R. and {Perry}, M.},
        ADDRESS = "ESA SP-419"}


@ARTICLE{Castelli1994A&A...281..817C,
    author = {{Castelli}, F. and {Kurucz}, R.~L.},
    title = "{Model atmospheres for VEGA}",
    journal = {\aap},
    year = 1994,
    month = jan,
    volume = 281,
    pages = {817--832},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1994A%26A...281..817C&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Cayrel1985A&A...146..249C,
    author = {{Cayrel}, R. and {Cayrel de Strobel}, G. and {Campbell}, B.},
    title = "Steps towards the abundance scale. I - The abundance of heavy elements in the Hyades cluster",
    journal = {\aap},
    year = 1985,
    month = may,
    volume = 146,
    pages = {249--259},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1985A%26A...146..249C&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Cayrel1992A&AS...95..273C,
    author = {{Cayrel de Strobel}, G. and {Hauck}, B. and {Francois}, P. and 
        {Thevenin}, F. and {Friel}, E. and {Mermilliod}, M. and {Borde}, S.
        },
    title = "{A catalogue of Fe/H determinations - 1991 edition}",
    journal = {\aaps},
    year = 1992,
    month = oct,
    volume = 95,
    pages = {273--336},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1992A%26AS...95..273C&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Charbonnel1994A&A...282..811C,
    author = {{Charbonnel}, C.},
    title = "Clues for non-standard mixing on the red giant branch from C-12/C-13 and C-12/N-14 ratios in evolved stars",
    journal = {\aap},
    year = 1994,
    month = feb,
    volume = 282,
    pages = {811--820},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1994A%26A...282..811C&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Charbonnel1995ApJ...453L..41C,
    author = {{Charbonnel}, C.},
    title = "A Consistent Explanation for 12C/ 13C, 7Li and 3He Anomalies in Red Giant Stars",
    journal = {\apjl},
    year = 1995,
    month = nov,
    volume = 453,
    pages = {L41},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1995ApJ...453L..41C&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Charbonnel1998A&A...332..204C,
    author = {{Charbonnel}, C. and {Brown}, J.\ A. and {Wallerstein}, G.},
    title = "Mixing processes during the evolution of red giants with moderate metal deficiencies: the role of molecular-weight barriers",
    journal = {\aap},
    year = 1998,
    month = apr,
    volume = 332,
    pages = {204--214},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1998A%26A...332..204C&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Chmielewski1992A&A...263..219C,
    author = {{Chmielewski}, Y. and {Friel}, E. and {Cayrel de Strobel}, G. and 
        {Bentolila}, C.},
    title = {The 1992 detailed analyses of Alpha Centauri A and Alpha Centauri B},
    journal = {\aap},
    year = 1992,
    month = sep,
    volume = 263,
    pages = {219--231},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1992A%26A...263..219C&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Ciardi2001ApJ...559.1147C,
    author = {{Ciardi}, D.~R. and {van Belle}, G.~T. and {Akeson}, R.~L. and 
        {Thompson}, R.~R. and {Lada}, E.~A. and {Howell}, S.~B.},
    title = "{On the Near-Infrared Size of Vega}",
    journal = {\apj},
    year = 2001,
    month = oct,
    volume = 559,
    pages = {1147--1154},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2001ApJ...559.1147C&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Claret1995A&AS..114..549C,
    author = {{Claret}, A. and {Gimenez}, A.},
    title = "Stellar models for a wide range of initial chemical compositions until helium burning. II. From X=0.63 to X=0.80, for Z=0.01.",
    journal = {\aaps},
    year = 1995,
    month = dec,
    volume = 114,
    pages = {549},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1995A%26AS..114..549C&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Clegg1979ApJ...234..188C,
    author = {{Clegg}, R.\ E.\ S. and {Lambert}, D.\ L. and {Bell}, R.\ A.
        },
    title = "Isotopes of titanium in cool stars",
    journal = {\apj},
    year = 1979,
    month = nov,
    volume = 234,
    pages = {188--199},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1979ApJ...234..188C&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{Code1976ApJ...203..417C,
    author = {{Code}, A.\ D. and {Bless}, R.\ C. and {Davis}, J. and {Brown}, R.\ H.
        },
    title = {Empirical effective temperatures and bolometric corrections for early-type stars},
    journal = {\apj},
    year = 1976,
    month = jan,
    volume = 203,
    pages = {417--434},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1976ApJ...203..417C&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Cohen1992AJ....104.1650C,
    author = {{Cohen}, M. and {Walker}, R.\ G. and {Barlow}, M.\ J. and {Deacon}, J.\ R.
        },
    title = "Spectral irradiance calibration in the infrared. I - Ground-based and IRAS broadband calibrations",
    journal = {\aj},
    year = 1992,
    month = oct,
    volume = 104,
    pages = {1650--1657},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1992AJ....104.1650C&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Cohen1992AJ....104.2030C,
    author = {{Cohen}, M. and {Walker}, R.\ G. and {Witteborn}, F.\ C.},
    title = {Spectral irradiance calibration in the infrared. II - Alpha Tau
                  and the recalibration of the IRAS low resolution
                  spectrometer}, 
    journal = {\aj},
    year = 1992,
    month = nov,
    volume = 104,
    pages = {2030--2044},
    url =   {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1992AJ....104.2030C&db_key=AST}, 
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Cohen1995AJ....110..275C,
    author = {{Cohen}, M. and {Witteborn}, F.\ C. and {Walker}, R.\ G. and 
        {Bregman}, J.\ D. and {Wooden}, D.\ H.},
    title = {Spectral Irradiance Calibration in the Infrared.IV. 1.2-35 micron spectra of six standard stars},
    journal = {\aj},
    year = 1995,
    month = jul,
    volume = 110,
    pages = {275},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1995AJ....110..275C&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Cohen1996AJ....112..241C,
    author = {{Cohen}, M. and {Witteborn}, F.\ C. and {Bregman}, J.\ D. and 
        {Wooden}, D.\ H. and {Salama}, A. and {Metcalfe}, L.},
    title = {Spectral Irradiance Calibration in the Infrared. VI. 3-35 micron Spectra of Three Southern Standard Stars},
    journal = {\aj},
    year = 1996,
    month = jul,
    volume = 112,
    pages = {241},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1996AJ....112..241C&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Cohen1996AJ....112.2274C,
    author = {{Cohen}, M. and {Witteborn}, F.\ C. and {Carbon}, D.\ F. and 
        {Davies}, J.\ K. and {Wooden}, D.\ H. and {Bregman}, J.\ D.},
    title = {Spectral Irradiance Calibration in the Infrared.VII.New Composite Spectra, Comparison with Model Atmospheres, and Far-Infrared Extrapolations},
    journal = {\aj},
    year = 1996,
    month = nov,
    volume = 112,
    pages = {2274},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1996AJ....112.2274C&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Cohen1999AJ....117.1864C,
    author = {{Cohen}, M. and {Walker}, R.\ G. and {Carter}, B. and {Hammersley}, P. and 
        {Kidger}, M. and {Noguchi}, K.},
    title = "Spectral Irradiance Calibration in the Infrared. X. A Self-Consistent Radiometric All-Sky Network of Absolutely Calibrated Stellar Spectra",
    journal = {\aj},
    year = 1999,
    month = apr,
    volume = 117,
    pages = {1864--1889},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1999AJ....117.1864C&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Cornide1992AJ....103.1374C,
    author = {{Cornide}, M. and {Fernandez-Figueroa}, M.\ J. and {de Castro}, E. and 
        {Armentia}, J.\ A. and {Reglero}, V.},
    title = "Stellar activity in barium stars. I - Analysis of H and K CA II lines in ten barium stars",
    journal = {\aj},
    year = 1992,
    month = apr,
    volume = 103,
    pages = {1374--1380},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1992AJ....103.1374C&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Cousins1972MNSSA..31...69C,
    author = {{Cousins}, A.~W.~J.},
    title = "{UBV photometry of some very bright stars}",
    journal = {Monthly Notes of the Astronomical Society of South Africa},
    year = 1972,
    volume = 31,
    pages = {69},
    url = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1972MNSSA..31...69C&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Currie1974ApJ...187..131C,
    author = {{Currie}, D.~G. and {Knapp}, S.~L. and {Liewer}, K.~M.},
    title = "{Four stellar-diameter measurements by a new technique : amplitude interferometry.}",
    journal = {\apj},
    year = 1974,
    month = jan,
    volume = 187,
    pages = {131--134},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1974ApJ...187..131C&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@INPROCEEDINGS{Davis1998IAUS..189...31D,
    author = {{Davis}, J.},
    title = "{Stellar angular diameter measurements by interferometry}",
    booktitle = {IAU Symp. 189: Fundamental Stellar Properties},
    year = 1998,
    volume = 189,
    pages = {31},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1998IAUS..189...31D&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}



@ARTICLE{Dearborn1976ApJ...203..455D,
    author = {{Dearborn}, D.~S.~P. and {Eggleton}, P.~P. and {Schramm}, D.~N.
        },
    title = "{12C/13C ratios in stars ascending the giant branch the first time.}",
    journal = {\apj},
    year = 1976,
    month = jan,
    volume = 203,
    pages = {455--462},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1976ApJ...203..455D&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Dearborn1975ApJ...200..675D,
    author = {{Dearborn}, D.\ S.\ P. and {Lambert}, D.\ L. and {Tomkin}, J.
        },
    title = "The C-12/C-13 ratio in stellar atmospheres. V - Twelve K giants and subgiants",
    journal = {\apj},
    year = 1975,
    month = sep,
    volume = 200,
    pages = {675--681},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1975ApJ...200..675D&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}



@ARTICLE{Decat2000A&A...355.1015D,
    author = {{De Cat}, P. and {Aerts}, C. and {De Ridder}, J. and {Kolenberg},
                  K. and  {Meeus}, G. and {Decin}, L.},
    title = {A study of bright southern slowly pulsating B
                  stars. I. Determination of the orbital parameters and of the
                  main frequency  of the spectroscopic binaries}, 
    journal = {\aap},
    year = 2000,
    month = mar,
    volume = 355,
    pages = {1015--1030},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2000A%26A...355.1015D&db_key=AST}, 
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@INPROCEEDINGS{Decin1997fiso.work..185D,
    author = {{Decin}, L. and {Cohen}, M. and {Eriksson}, K. and {Gustafsson}, B. and 
        {Huygen}, E. and {Morris}, P. and {Plez}, B. and {Sauval}, J. and 
        {Vandenbussche}, B. and {Waelkens}, C.},
    title = {Comparison Bertween ISO-SWS Observations and Synthetic Spectra of K Giants and M Giants: $\alpha$ Boo and {\&} $\beta$ Peg},
    booktitle = {The first ISO workshop on Analytical Spectroscopy},
    year = 1997,
    pages = {185},
      EDITOR    = {{Heras}, A.\ M. and {Leech}, K. and {Trams}, N.\ R. and {Perry}, M.},
        ADDRESS = "ESA SP-419"}




@PHDTHESIS{Decinthesis,
    author = {{Decin}, L.},
    title = {Synthetic spectra of cool stars observed with the Short-Wavelength Spectrometer: improving the models and the calibration of the instrument},
    school = {University of Leuven},
    year = 2000,
}

@ARTICLE{Decin2000A&A...364..137D,
    author = {{Decin}, L. and {Waelkens}, C. and {Eriksson}, K. and {Gustafsson}, B. and 
        {Plez}, B. and {Sauval}, A.\ J. and {Van Assche}, W. and
                  {Vandenbussche}, B. 
        }, 
    title = "ISO-SWS calibration and the accurate modelling  of
                  cool-star atmospheres. I.\ Method", 
    journal = {\aap},
    year = 2000,
    month = dec,
    volume = 364,
    pages = {137--156},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2000A%26A...364..137D&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{Decin2000b,
         author = {{Decin}, L.  and {Vandenbussche}, B. and
                  {Waelkens}, C. and {Eriksson}, K. and  
                  {Gustafsson}, B. and {Plez}, B. and {Sauval}, A.\ J. and {Van
                  Assche}, W.},  
        TITLE   = "ISO-SWS calibration and the accurate modelling of cool-star
                  atmospheres: II.\ Results", 
        YEAR    = 2002,
        JOURNAL = aa,
        VOLUME  = {in press},
        PAGES   = {(Paper~II)}
}

@ARTICLE{Decin2000c,
         author = {{Decin}, L.  and {Vandenbussche}, B. and
                  {Waelkens}, C. and {Eriksson}, K. and 
                  {Gustafsson}, B. and {Plez}, B. and {Sauval}, A.\ J. and {Van
                  Assche}, W.},  
        TITLE   = "ISO-SWS calibration and the accurate modelling of cool-star
                  atmospheres: III.\ A0 to G2 stars", 
        YEAR    = 2002,
        JOURNAL = aa,
        VOLUME  = {in press},
        PAGES   = {(Paper~III)}
}

@ARTICLE{Decin2000d,
         author = {{Decin}, L.  and {Vandenbussche}, B. and
                  {Waelkens}, C. and {Eriksson}, K. and 
                  {Gustafsson}, B. and {Plez}, B. and {Sauval}, A.\ J. and {Van
                  Assche}, W.},  
        TITLE   = "ISO-SWS calibration and the accurate modelling of cool-star
                  atmospheres: IV.\ G9 to M2 stars", 
        YEAR    = 2002,
        JOURNAL = aa,
        VOLUME  = {in press},
        PAGES   = {(Paper~IV)}
}

@ARTICLE{Decin2000e,
         author = {{Decin}, L.  and {Vandenbussche}, B. and
                  {Waelkens}, C. and {Eriksson}, K. and 
                  {Gustafsson}, B. and {Plez}, B. and {Sauval}, A.\ J. and {Van
                  Assche}, W.},  
        TITLE   = "ISO-SWS calibration and the accurate modelling of cool-star
                  atmospheres: V.\ ", 
        YEAR    = 2002,
        JOURNAL = aa,
        VOLUME  = {in prep.},
        PAGES   = {}
}



@ARTICLE{deGraauw1996A&A...315L..49D,
    author = {{de Graauw}, T. and {Haser}, L.\ N. and {Beintema}, D.\ A. and 
        {Roelfsema}, P.\ R. and {van Agthoven}, H. and {Barl}, L. and 
        {Bauer}, O.\ H. and {Bekenkamp}, H.\ E.\ G. and {Boonstra}, A.\ -. and 
        {Boxhoorn}, D.\ R. and {Cote}, J. and {de Groene}, P. and {van Dijkhuizen}, C. and 
        {Drapatz}, S. and {Evers}, J. and {Feuchtgruber}, H. and {Frericks}, M. and 
        {Genzel}, R. and {Haerendel}, G. and {Heras}, A.\ M. and {van der Hucht}, K.\ A. and 
        {van der Hulst}, T. and {Huygen}, R. and {Jacobs}, H. and {Jakob}, G. and 
        {Kamperman}, T. and {Katterloher}, R.\ O. and {Kester}, D.\ J.\ M. and 
        {Kunze}, D. and {Kussendrager}, D. and {Lahuis}, F. and {Lamers}, H.\ J.\ G.\ L.\ M. and 
        {Leech}, K. and {van der Lei}, S. and {van der Linden}, R. and 
        {Luinge}, W. and {Lutz}, D. and {Melzner}, F. and {Morris}, P.\ W. and 
        {van Nguyen}, D. and {Ploeger}, G. and {Price}, S. and {Salama}, A. and 
        {Schaeidt}, S.\ G. and {Sijm}, N. and {Smoorenburg}, C. and 
        {Spakman}, J. and {Spoon}, H. and {Steinmayer}, M. and {Stoecker}, J. and 
        {Valentijn}, E.\ A. and {Vandenbussche}, B. and {Visser}, H. and 
        {Waelkens}, C. and {Waters}, L.\ B.\ F.\ M. and {Wensink}, J. and 
        {Wesselius}, P.\ R. and {Wiezorrek}, E. and {Wieprecht}, E. and 
        {Wijnbergen}, J.\ J. and {Wildeman}, K.\ J. and {Young}, E.},
    title = "Observing with the ISO Short-Wavelength Spectrometer.",
    journal = {\aap},
    year = 1996,
    month = nov,
    volume = 315,
    pages = {L49--L54},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1996A%26A...315L..49D&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@INPROCEEDINGS{deJong1999,                                       
        AUTHOR  = {{de Jong}, T.}, 
        TITLE   = "",
        BOOKTITLE = "Abstracts of the 2nd Austrian ISO
Workshop. Atmospheres of M, S and C Giants.",
        YEAR    = 1999,
        PAGES   = "53",
      EDITOR    = {{Hron}, J.  and {H{\"{o}}fner}, S.},
        ADDRESS = ""}



@ARTICLE{Demarque1986ApJ...300..773D,
    author = {{Demarque}, P. and {Guenther}, D.\ B. and {van Altena}, W.\ F.
        },
    title = {The case of Alpha Centauri - Mass, age and p-mode oscillation spectrum},
    journal = {\apj},
    year = 1986,
    month = jan,
    volume = 300,
    pages = {773--778},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1986ApJ...300..773D&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Desikachary1982MNRAS.201..707D,
    author = {{Desikachary}, K. and {Hearnshaw}, J.\ B.},
    title = {The spectrum of Canopus. II - Analysis and composition},
    journal = {\mnras},
    year = 1982,
    month = nov,
    volume = 201,
    pages = {707--721},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1982MNRAS.201..707D&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{DiBenedetto1987A&A...188..114D,
    author = {{di Benedetto}, G.\ P. and {Rabbia}, Y.},
    title = {Accurate angular diameters and effective temperatures for eleven giants cooler than K0 by Michelson interferometry},
    journal = {\aap},
    year = 1987,
    month = dec,
    volume = 188,
    pages = {114--124},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1987A%26A...188..114D&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{DiBenedetto1993A&A...270..315D,
    author = {{di Benedetto}, G.~P.},
    title = "{Empirical effective temperatures and angular diameters of stars cooler than the sun}",
    journal = {\aap},
    year = 1993,
    month = mar,
    volume = 270,
    pages = {315--334},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1993A%26A...270..315D&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}



@ARTICLE{DiBenedetto1998A&A...339..858D,
    author = {{di Benedetto}, G.\ P.},
    title = "Towards a fundamental calibration of stellar parameters  of A, F, G, K dwarfs and giants",
    journal = {\aap},
    year = 1998,
    month = nov,
    volume = 339,
    pages = {858--871},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1998A%26A...339..858D&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Dreiling1980ApJ...241..736D,
    author = {{Dreiling}, L.\ A. and {Bell}, R.\ A.},
    title = "The chemical composition, gravity, and temperature of VEGA",
    journal = {\apj},
    year = 1980,
    month = oct,
    volume = 241,
    pages = {736--758},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1980ApJ...241..736D&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Drira1997A&A...319..720D,
    author = {{Drira}, I. and {Hure}, J.\ M. and {Spielfiedel}, A. and {Feautrier}, N. and 
        {Roueff}, E.},
    title = "Infrared transitions probabilities and radiative opacity of SiO.",
    journal = {\aap},
    year = 1997,
    month = mar,
    volume = 319,
    pages = {720--724},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1997A%26A...319..720D&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Dyck1974ApJ...189...89D,
    author = {{Dyck}, H.\ M. and {Lockwood}, G.\ W. and {Capps}, R.\ W.},
    title = "Infrared fluxes spectral types and temperatures for very cool stars.",
    journal = {\apj},
    year = 1974,
    month = apr,
    volume = 189,
    pages = {89--100},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1974ApJ...189...89D&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Dyck1998AJ....116..981D,
    author = {{Dyck}, H.\ M. and {van Belle}, G.\ T. and {Thompson}, R.\ R.
        },
    title = "Radii and Effective Temperatures for K and M Giants and Supergiants. II.",
    journal = {\aj},
    year = 1998,
    month = aug,
    volume = 116,
    pages = {981--986},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1998AJ....116..981D&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Edvardsson1988A&A...190..148E,
    author = {{Edvardsson}, B.},
    title = {Spectroscopic surface gravities and chemical compositions for 8 nearby single sub-giants},
    journal = {\aap},
    year = 1988,
    month = jan,
    volume = 190,
    pages = {148--166},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1988A%26A...190..148E&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Eggen1973PASP...85..379E,
    author = {{Eggen}, O.\ J.},
    title = "Luminosity and velocity distribution of high-luminosity stars near the sun. II. The young disk giants",
    journal = {\pasp},
    year = 1973,
    month = aug,
    volume = 85,
    pages = {379--395},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1973PASP...85..379E&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{ElEid1994A&A...285..915E,
    author = {{El Eid}, M.\ F.},
    title = {CNO isotopes in red giants: theory versus observations},
    journal = {\aap},
    year = 1994,
    month = may,
    volume = 285,
    pages = {915--928},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1994A%26A...285..915E&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Engelke1992AJ....104.1248E,
    author = {{Engelke}, C.\ W.},
    title = {Analytic approximations to the 2-60 microns infrared continua for standard calibration stars - With application to the calibration of spectroscopy and photometry, and the determination of effective temperature and angular size from IR measurements},
    journal = {\aj},
    year = 1992,
    month = sep,
    volume = 104,
    pages = {1248--1259},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1992AJ....104.1248E&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{England1980MNRAS.191...23E,
    author = {{England}, M.\ N.},
    title = {A spectroscopic analysis of the Alpha Centauri system},
    journal = {\mnras},
    year = 1980,
    month = apr,
    volume = 191,
    pages = {23--35},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1980MNRAS.191...23E&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Fagotto1994A&AS..105...29F,
    author = {{Fagotto}, F. and {Bressan}, A. and {Bertelli}, G. and {Chiosi}, C.
        },
    title = "{Evolutionary sequences of stellar models with new radiative opacities. IV. Z=0.004 and Z=0.008}",
    journal = {\aaps},
    year = 1994,
    month = may,
    volume = 105,
    pages = {29--38},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1994A%26AS..105...29F&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@BOOK{Farmer1989QB551.F37......,
    author = {{Farmer}, C.\ B. and {Norton}, R.\ H.},
    title = {A High-Resolution Atlas of the Infrared Spectrum of the Sun and
                  Earth Atmosphere from Space.  Volume I. The Sun}, 
    publisher = {Washington, D.C.\ : NASA, Scientific and Technical Information Division},  
    year = 1989,
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1989QB551.F37......&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Faucherre1983A&A...120..263F,
    author = {{Faucherre}, M. and {Bonneau}, D. and {Koechlin}, L. and {Vakili}, F.
        },
    title = "Stellar interferometry - Diameters and effective temperatures of five giant stars",
    journal = {\aap},
    year = 1983,
    month = apr,
    volume = 120,
    pages = {263--268},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1983A%26A...120..263F&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Fernandez-Villacanas1990AJ.....99.1961F,
    author = {{Fern\'{a}ndez-Villaca\~{n}as}, J.\ L. and {Rego}, M. and {Cornide}, M.
        },
    title = "Barium and iron abundances in red giants",
    journal = {\aj},
    year = 1990,
    month = jun,
    volume = 99,
    pages = {1961--1970},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1990AJ.....99.1961F&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@BOOK{Feuchtgruber1998,
        AUTHOR  = "{Feuchtgruber}, H.",
        TITLE   = {Status of AOT01 AOT band order ratios
                    and related data}, 
      PUBLISHER = {ISO-SWS online documentation},
        YEAR    = 1998}

@ARTICLE{Flannery1978ApJ...221..175F,
    author = {{Flannery}, B.\ P. and {Ayres}, T.\ R.},
    title = {Evolution of the Alpha Centauri system},
    journal = {\apj},
    year = 1978,
    month = apr,
    volume = 221,
    pages = {175--185},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1978ApJ...221..175F&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Flower1996ApJ...469..355F,
    author = {{Flower}, P.\ J.},
    title = "Transformations from Theoretical Hertzsprung-Russell Diagrams to Color-Magnitude Diagrams: Effective Temperatures, B-V Colors, and Bolometric Corrections",
    journal = {\apj},
    year = 1996,
    month = sep,
    volume = 469,
    pages = {355},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1996ApJ...469..355F&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Flynn1991A&A...250..400F,
    author = {{Flynn}, C. and {Mermilliod}, J.\ -.},
    title = "On the DDO absolute magnitudes of K giants",
    journal = {\aap},
    year = 1991,
    month = oct,
    volume = 250,
    pages = {400--406},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1991A%26A...250..400F&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}



@ARTICLE{Fracassini1988BICDS..35..121F,
    author = {{Fracassini}, M. and {Pasinetti-Fracassini}, L.\ E. and {Pastori}, L. and 
        {Pironi}, R.},
    title = {Catalogue of Apparent Diameters and Absolute Radii of Stars},
    journal = {Bulletin d'Information du Centre de Donnees Stellaires},
    year = 1988,
    month = dec,
    volume = 35,
    pages = {121},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1988BICDS..35..121F&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Frisk1982MNRAS.199..471F,
    author = {{Frisk}, U. and {Nordh}, H.\ L. and {Olofsson}, S.\ G. and {Bell}, R.\ A. and 
        {Gustafsson}, B.},
    title = "The temperature of Arcturus",
    journal = {\mnras},
    year = 1982,
    month = may,
    volume = 199,
    pages = {471--481},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1982MNRAS.199..471F&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@BOOK{Fuhr1988atps.book.....F, 
    author = {{Fuhr}, J.\ R. and {Martin}, G.\ A. and {Wiese}, W.\ L.},
    title = {Atomic transition probabilities. Scandium through Manganese},
    publisher = {New York: American Institute of Physics (AIP) and American Chemical Society}, 
    year = 1988,
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1988atps.book.....F&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@BOOK{Fuhr1988atpi.book.....F,
    author = {{Fuhr}, J.\ R. and {Martin}, G.\ A. and {Wiese}, W.\ L.},
    title = {Atomic transition probabilities. Iron through Nickel},
    publisher = {New York: American Institute of Physics (AIP) and American Chemical Society},
    year = 1988,
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1988atpi.book.....F&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Furenlid1990ApJ...350..827F,
    author = {{Furenlid}, I. and {Meylan}, T.},
    title = {An abundance analysis of Alpha Centauri A},
    journal = {\apj},
    year = 1990,
    month = feb,
    volume = 350,
    pages = {827--838},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1990ApJ...350..827F&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Johnson1966ARA&A...4..193J,
    author = {{Johnson}, H.~L.},
    title = "{Astronomical Measurements in the Infrared}",
    journal = {\araa},
    year = 1966,
    volume = 4,
    pages = {193},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1966ARA%26A...4..193J&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}



@ARTICLE{Judge1986MNRAS.221..119J,
    author = {{Judge}, P.\ G.},
    title = "Constraints on the outer atmospheric structure of late-type giant stars with IUE - Methods and application to Arcturus (Alpha Boo K2III)",
    journal = {\mnras},
    year = 1986,
    month = jul,
    volume = 221,
    pages = {119--153},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1986MNRAS.221..119J&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Judge1991ApJ...371..357J,
    author = {{Judge}, P.\ G. and {Stencel}, R.\ E.},
    title = "Evolution of the chromospheres and winds of low- and intermediate-mass giant stars",
    journal = {\apj},
    year = 1991,
    month = apr,
    volume = 371,
    pages = {357--379},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1991ApJ...371..357J&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Gadun1994AN....315..413G,
    author = {{Gadun}, A.\ S.},
    title = {Iron abundance and microturbulence in Arcturus, Canopus, alpha CEN A, and Sun from FeI and FeII lines},
    journal = {Astronomische Nachrichten},
    year = 1994,
    month = dec,
    volume = 315,
    pages = {413--418},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1994AN....315..413G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Gardiner1999A&A...347..876G,
    author = {{Gardiner}, R.~B. and {Kupka}, F. and {Smalley}, B.},
    title = "{Testing convection theories using Balmer line profiles of A, F, and G stars}",
    journal = {\aap},
    year = 1999,
    month = jul,
    volume = 347,
    pages = {876--890},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1999A%26A...347..876G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@BOOK{Geller1992,
    author = {{Geller}, M.},
    title = {A High-Resolution Atlas of the Infrared Spectrum of the Sun and
                  Earth Atmosphere from Space. Volume III. Key to Identification
                  of Solar Features},
    publisher = {Washington, D.C.\ : NASA, Scientific and Technical Information                  Division},   
    year = 1992,
    url = {},
}

@ARTICLE{Gezari1972ApJ...173L...1G,
    author = {{Gezari}, D.~Y. and {Labeyrie}, A. and {Stachnik}, R.~V.},
    title = "{Speckle Interferometry: Diffraction-Limited Measurements of Nine Stars with the 200-INCH Telescope}",
    journal = {\apjl},
    year = 1972,
    month = apr,
    volume = 173,
    pages = {L1},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1972ApJ...173L...1G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Gezari1999yCat.2225....0G,
    author = {{Gezari}, D.~Y. and {Pitts}, P.~S. and {Schmitz}, M.},
    title = "{Catalog of Infrared Observations, Edition 5 (Gezari+ 1999)}",
    journal = {VizieR Online Data Catalog},
    year = 1999,
    month = jul,
    volume = 2225,
    pages = {0},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1999yCat.2225....0G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Gigas1986A&A...165..170G,
    author = {{Gigas}, D.},
    title = "The iron abundance of VEGA",
    journal = {\aap},
    year = 1986,
    month = sep,
    volume = 165,
    pages = {170--182},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1986A%26A...165..170G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Girardi2000A&AS..141..371G,
    author = {{Girardi}, L. and {Bressan}, A. and {Bertelli}, G. and {Chiosi}, C.
        },
    title = "Evolutionary tracks and isochrones for low- and intermediate-mass stars: From 0.15 to 7 M$_{\odot}$, and from Z=0.0004 to 0.03",
    journal = {\aaps},
    year = 2000,
    month = feb,
    volume = 141,
    pages = {371--383},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2000A%26AS..141..371G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Glass1974MNSSA..33...53G,
    author = {{Glass}, I.~S.},
    title = "{JHKL photometry of 145 southern stars.}",
    journal = {Monthly Notes of the Astronomical Society of South Africa},
    year = 1974,
    volume = 33,
    pages = {53--58},
    url = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1974MNSSA..33...53G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Glebocki1988A&A...189..199G,
    author = {{Glebocki}, R. and {Stawikowski}, A.},
    title = "Are tides responsible for enhanced MG II emission in late-type binaries?",
    journal = {\aap},
    year = 1988,
    month = jan,
    volume = 189,
    pages = {199--203},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1988A%26A...189..199G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Gliese1969VeARI..22....1G,
    author = {{Gliese}, W.},
    title = {Catalogue of Nearby Stars. Edition 1969},
    journal = {Ver\"{o}ffentlichungen des Astronomishen Rechen-Instituts Heidelberg},
    year = 1969,
    volume = 22,
    pages = {1},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1969VeARI..22....1G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}



@ARTICLE{Goldman1998,
        AUTHOR  = "{Goldman}, A. and {Schoenfeld}, W.\ G. and {Goorvitch},
                  D. and {Chackerian}, C.\ Jr. and {Dothe} H. and {M\'{e}len},
                  F. and {Abrams}, M.\ C. and {Selby}, J.\ E.\ A.",
        TITLE   = "Updated line parameters for OH X$^2\Pi$-X$^2\Pi$
                  $(v\prime\prime,v\prime)$ transitions",
        YEAR    = 1998,
        JOURNAL = jqsrt,
        VOLUME  = 59,
        PAGES   = "453--469"}



@ARTICLE{Gratton1982MNRAS.201..807G,
    author = {{Gratton}, L. and {Gaudenzi}, S. and {Rossi}, C. and {Gratton}, R.\ G.
        },
    title = "Studies on the spectra of K-giants. I - Physical parameters and Fe and Ti abundances for 26 K-giants",
    journal = {\mnras},
    year = 1982,
    month = dec,
    volume = 201,
    pages = {807--832},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1982MNRAS.201..807G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Gratton1983MNRAS.202..231G,
    author = {{Gratton}, R.\ G.},
    title = "Studies on the spectra of K-giants. II - Abundance determinations for K-giants from very strong iron lines",
    journal = {\mnras},
    year = 1983,
    month = jan,
    volume = 202,
    pages = {231--240},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1983MNRAS.202..231G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Gratton1985A&A...148..105G,
    author = {{Gratton}, R.\ G.},
    title = "Studies on the spectra of K-giants. III - Carbon, nitrogen, and oxygen abundances",
    journal = {\aap},
    year = 1985,
    month = jul,
    volume = 148,
    pages = {105--114},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1985A%26A...148..105G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Gray1975ApJ...202..148G,
    author = {{Gray}, D.\ F.},
    title = {Atmospheric turbulence measured in stars above the main sequence},
    journal = {\apj},
    year = 1975,
    month = nov,
    volume = 202,
    pages = {148--164},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1975ApJ...202..148G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@BOOK{Gray1992,
    author = {{Gray}, D.\ F.},
    title = {The observation and analysis of stellar photospheres},
    publisher = {Cambridge Astrophysics Series, Cambridge: Cambridge University Press, 1992, 2nd ed., ISBN 0521403200.},
    year = 1992,
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1992oasp.book.....G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Grevesse1992RMxAA..23...71G,
    author = {{Grevesse}, N. and {Sauval}, A.\ J.},
    title = "Molecular Data from Solar Spectroscopy",
    journal = {Revista Mexicana de Astronomia y Astrofisica, vol.\ 23},
    year = 1992,
    month = mar,
    volume = 23,
    pages = {71},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1992RMxAA..23...71G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@BOOK{Griffin1968,
    author = {{Griffin}, R.},
    title = "A photometric atlas of the spectrum of Arcturus, $\lambda \lambda 3600-8825$ {\AA}", 
    publisher = {Cambridge: Cambridge Philosophical Society, 1968},
    year = 1968,
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1968pmas.book.....G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Gunson1996GeoRL..23.2333G,
    author = {{Gunson}, M.\ R. and {Abbas}, M.\ M. and {Abrams}, M.\ C. and 
        {Allen}, M. and {Brown}, L.\ R. and {Brown}, T.\ L. and {Chang}, A.\ Y. and 
        {Goldman}, A. and {Irion}, F.\ W. and {Lowes}, L.\ L. and {Mahieu}, E. and 
        {Manney}, G.\ L. and {Michelsen}, H.\ A. and {Newchurch}, M.\ J. and 
        {Rinsland}, C.\ P. and {Salawitch}, R.\ J. and {Stiller}, G.\ P. and 
        {Toon}, G.\ C. and {Yung}, Y.\ L. and {Zander}, R.},
    title = "The atmospheric trace molecule spectroscopy (ATMOS) experiment: Deployment on the ATLAS Space Shuttle missions",
    journal = {\grl},
    year = 1996,
    volume = 23,
    pages = {2333},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1996GeoRL..23.2333G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Gustafsson1974A&A....34...99G,
    author = {{Gustafsson}, B. and {Kj{\ae}rgaard}, P. and {Andersen}, S.},
    title = "The metal content and microturbulence in G8-K3 giants, as investigated by means of photoelectric photometry in very narrow bands.",
    journal = {\aap},
    year = 1974,
    month = aug,
    volume = 34,
    pages = {99--128},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1974A%26A....34...99G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Gustafsson1975A&A....42..407G,
    author = {{Gustafsson}, B. and {Bell}, R.\ A. and {Eriksson}, K. and {Nordlund}, {\AA}.
        },
    title = {A grid of model atmospheres for metal-deficient giant stars. I},
    journal = {\aap},
    year = 1975,
    month = sep,
    volume = 42,
    pages = {407--432},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1975A%26A....42..407G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Gustafsson1979A&A....74..313G,
    author = {{Gustafsson}, B. and {Bell}, R.~A.},
    title = "{The colours of G and K type giant stars. I}",
    journal = {\aap},
    year = 1979,
    month = may,
    volume = 74,
    pages = {313--352},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1979A%26A....74..313G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Gustafsson1994A&ARv...6...19G,
    author = {{Gustafsson}, B. and {Jorgensen}, U.\ G.},
    title = "Models of late-type stellar photospheres",
    journal = {\aapr},
    year = 1994,
    month = nov,
    volume = 6,
    pages = {19--65},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1994A%26ARv...6...19G&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Hammersley1998A&AS..128..207H,
    author = {{Hammersley}, P.\ L. and {Jourdain de Muizon}, M. and {Kessler}, M.\ F. and 
        {Bouchet}, P. and {Joseph}, R.\ D. and {Habing}, H.\ J. and 
        {Salama}, A. and {Metcalfe}, L.},
    title = "Infrared standards for ISO. I. A new calibration of mid infrared photometry",
    journal = {\aaps},
    year = 1998,
    month = feb,
    volume = 128,
    pages = {207--219},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1998A%26AS..128..207H&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@INPROCEEDINGS{Hammersley2001clim.confE..23H,
    author = {{Hammersley}, P.},
    title = "Development of Stellar Photometric Standards for ISO.",
    booktitle = {The calibration legacy of the {ISO} Mission},
    year = 2001,
    pages = {to be published},
    EDITOR    =  {{Metcalfe}, L. and {Kessler}, M.\ F.\ K.},   
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Harris1984ApJ...285..674H,
    author = {{Harris}, M.\ J. and {Lambert}, D.\ L.},
    title = "Oxygen isotopic abundances in the atmospheres of seven red giant stars",
    journal = {\apj},
    year = 1984,
    month = oct,
    volume = 285,
    pages = {674--682},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1984ApJ...285..674H&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Harris1988ApJ...325..768H,
    author = {{Harris}, M.\ J. and {Lambert}, D.\ L. and {Smith}, V.\ V.},
    title = "Oxygen isotopic abundances in evolved stars. IV - Five K giants",
    journal = {\apj},
    year = 1988,
    month = feb,
    volume = 325,
    pages = {768--775},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1988ApJ...325..768H&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Harwit2001ApJ...557..844H,
    author = {{Harwit}, M. and {Malfait}, K. and {Decin}, L. and {Waelkens}, C. and 
        {Feuchtgruber}, H. and {Melnick}, G.~J.},
    title = "{The Infrared Continuum Spectrum of VY Canis Majoris}",
    journal = {\apj},
    year = 2001,
    month = aug,
    volume = 557,
    pages = {844--853},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2001ApJ...557..844H&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Hill1993A&A...276..142H,
    author = {{Hill}, G.\ M. and {Landstreet}, J.\ D.},
    title = "Compositional Differences among the A-Type Stars - Part One - Six Narrowlined Stars",
    journal = {\aap},
    year = 1993,
    month = sep,
    volume = 276,
    pages = {142},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1993A%26A...276..142H&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Hill1995A&A...293..347H,
    author = {{Hill}, V. and {Andrievsky}, S. and {Spite}, M.},
    title = {Chemical evolution of the Magellanic Clouds. VI. Chemical composition of nine F supergiants from different regions of the large Magellanic Cloud.},
    journal = {\aap},
    year = 1995,
    month = jan,
    volume = 293,
    pages = {347--359},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1995A%26A...293..347H&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Hinkle1982ApJ...252..697H,
    author = {{Hinkle}, K.\ H. and {Hall}, D.\ N.\ B. and {Ridgway}, S.\ T.
        },
    title = "Time series infrared spectroscopy of the Mira variable Chi Cygni",
    journal = {\apj},
    year = 1982,
    month = jan,
    volume = 252,
    pages = {697--714},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1982ApJ...252..697H&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Hinkle1995PASP..107.1042H,
    author = {{Hinkle}, K. and {Wallace}, L. and {Livingston}, W.},
    title = {Infrared Atlas of the Arcturus Spectrum, 0.9-5.3 microns},
    journal = {\pasp},
    year = 1995,
    month = nov,
    volume = 107,
    pages = {1042},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1995PASP..107.1042H&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@BOOK{Hinkle1995,
        AUTHOR  = {{Hinkle}, K. and {Wallace}, L. and {Livingston}, W.},
        TITLE   = "Infrared Atlas of the Arcturus Spectrum, 0.9 -- 5.3 microns",
      PUBLISHER = "ASP, San Francisco",
        YEAR    = 1995
}




@BOOK{Hirhor95,
        AUTHOR  = {{Hirata}, R. and {Horaguchi}, T.},
        TITLE   = "Atomic spectral line list",
      PUBLISHER = "{internet: http://cdsweb.u-strasbg.fr/htbin/Cat?VI/69}",
        YEAR    = 1995,
        ADDRESS = ""}

@BOOK{Hoffleit1982,
    author = {{Hoffleit}, D. and {Jaschek}, C.},
    title = {The Bright Star Catalogue},
    publisher = {The Bright Star Catalogue, New Haven: Yale University Observatory (4th edition), 1982 },
    year = 1982,
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1982bsc..book.....H&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@INPROCEEDINGS{Hofner2001,                                       
        AUTHOR  = {{H\"{o}fner}, S. and {Loidl}, R. and {Aringer}, B. and {J{\o}rgensen}, U.}, 
        TITLE   = "Dynamical Atmospheres and Mass Loss of Pulsating AGB stars",
        BOOKTITLE = {ASP Conf. Ser.: Radial and Nonradial Pulsations as Probes of Stellar Physics},
        YEAR    = 2002,
        PAGES   = "{in press}",
      EDITOR    = "{Aerts}, C. and {Bedding}, T. and {Christensen-Dalsgaard}, J.",
      PUBLISHER = "{San Francisco: ASP}",
        ADDRESS = ""}


@ARTICLE{HolwegerMuller1974SoPh...39...19H,
    author = {{Holweger}, H. and {M\"{u}ller}, E.\ A.},
    title = {The photospheric barium spectrum - Solar abundance and collision broadening of BA II lines by hydrogen},
    journal = {\solphys},
    year = 1974,
    month = nov,
    volume = 39,
    pages = {19--30},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1974SoPh...39...19H&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Holweger1995A&A...303..819H,
    author = {{Holweger}, H. and {Rentzsch-Holm}, I.},
    title = {High-resolution spectroscopy of $\{$lambda$\}$ Bootis stars and `dusty' normal A stars: circumstellar gas, rotation, and accretion.},
    journal = {\aap},
    year = 1995,
    month = nov,
    volume = 303,
    pages = {819},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1995A%26A...303..819H&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Hui-Bon-Hoa1997A&A...323..901H,
    author = {{Hui-Bon-Hoa}, A. and {Burkhart}, C. and {Alecian}, G.},
    title = "Metal abundances of A-type stars in three galactic clusters.",
    journal = {\aap},
    year = 1997,
    month = jul,
    volume = 323,
    pages = {901--908},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1997A%26A...323..901H&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Hutter1989ApJ...340.1103H,
    author = {{Hutter}, D.\ J. and {Johnston}, K.\ J. and {Mozurkewich}, D. and 
        {Simon}, R.\ S. and {Colavita}, M.\ M. and {Pan}, X.\ P. and 
        {Shao}, M. and {Hines}, B.\ E. and {Staelin}, D.\ H. and {Hershey}, J.\ L. and 
        {Hughes}, J.\ A. and {Kaplan}, G.\ H.},
    title = "Angular diameter measurements of 24 giant and supergiant stars from the Mark III optical interferometer",
    journal = {\apj},
    year = 1989,
    month = may,
    volume = 340,
    pages = {1103--1111},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1989ApJ...340.1103H&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Iben1967ApJ...147..624I,
    author = {{Iben}, I.~J.},
    title = "{Stellar Evolution.VI. Evolution from the Main Sequence to the Red-Giant Branch for Stars of Mass 1 M\_$\{$sun$\}$, 1.25 M\_$\{$sun$\}$, and 1.5 M\_$\{$sun$\}$}",
    journal = {\apj},
    year = 1967,
    month = feb,
    volume = 147,
    pages = {624},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1967ApJ...147..624I&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@BOOK{Jenkins1952QB813.J45......,
    author = {{Jenkins}, L.\ F.},
    title = "General catalogue of trigonometric stellar parallaxes.",
    publisher = {New Haven, Yale University Observatory},
    year = 1952,
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1952QB813.J45......&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@INPROCEEDINGS{Jenkins1963GCTP..C......0J,
    author = {{Jenkins}, L.~F.},
    title = "{Supplement to the General Catalogue of Trigonometric Stellar Parallaxes, Compiled at the Yale Univ. Obs.}",
    booktitle = {General Cat. Trigo. Parallaxes (1963)},
    year = 1963,
    pages = {0},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1963GCTP..C......0J&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Johnson1966CoLPL...4...99J,
    author = {{Johnson}, H.~L. and {Iriarte}, B. and {Mitchell}, R.~I. and 
        {Wisniewskj}, W.~Z.},
    title = "{UBVRIJKL photometry of the bright stars.}",
    journal = {Communications of the Lunar and Planetary Laboratory},
    year = 1966,
    volume = 4,
    pages = {99},
    url = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1966CoLPL...4...99J&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}




@ARTICLE{Jorgensen1992A&A...261..263J,
    author = {{J{\o}rgensen}, U.\ G. and {Johnson}, H.\ R. and
                  {Nordlund}, {\AA}.},
    title = "Effects of sphericity in carbon star atmospheres",
    journal = {\aap},
    year = 1992,
    month = jul,
    volume = 261,
    pages = {263--273},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1992A%26A...261..263J&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@INPROCEEDINGS{Jorgensen1994mse..conf...29J,
    author = {{J{\o}rgensen}, U.\ G.},
    title = {Dominating Molecules in the Photosphere of Cool Stars},
    booktitle = {Molecules in the Stellar Environment, Proceedings of IAU Colloquium No. 146}, 
    year = 1994,
    pages = {29},
    EDITOR    = {{J{\o}rgensen}, U.\ G.},
        ADDRESS = "Springer-Verlag Berlin Heidelberg New York"}



@ARTICLE{Justtanont1998A&A...330L..17J,
    author = {{Justtanont}, K. and {Feuchtgruber}, H. and {de Jong}, T. and 
        {Cami}, J. and {Waters}, L.\ B.\ F.\ M. and {Yamamura}, I. and 
        {Onaka}, T.},
    title = "Discovery of CO\_2 emission in AGB stars  with the 13mu M dust feature",
    journal = {\aap},
    year = 1998,
    month = feb,
    volume = 330,
    pages = {L17--L20},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1998A%26A...330L..17J&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Kamper1978AJ.....83.1653K,
    author = {{Kamper}, K.\ W. and {Wesselink}, A.\ J.},
    title = {Alpha and Proxima Centauri},
    journal = {\aj},
    year = 1978,
    month = dec,
    volume = 83,
    pages = {1653--1659},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1978AJ.....83.1653K&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@BOOK{Kelly1983,
        AUTHOR  = "{Kelly}, R.\ L.",
        TITLE   = "Unpublished work",
        PUBLISHER = {magnetic tape},
        YEAR    = 1983,
        ADDRESS = ""}

@INPROCEEDINGS{Kester2001clim.confE..46K,
    author = {{Kester}, D. and {Fouks}, B. and {Lahuis}, F.},
    title = "{SWS Transient Effects: Models and Corrections}",
    booktitle = {The Calibration Legacy of the ISO Mission},
    year = 2001,
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2001clim.confE..46K&db_key=AST},
    PAGES   = {46},
    EDITOR    = {{Metcalfe}, L. and {Kessler}, F.\ K.},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Kjaergaard1982A&A...115..145K,
    author = {{Kj{\ae}rgaard}, P. and {Gustafsson}, B. and {Walker}, G.\ A.\ H. and 
        {Hultqvist}, L.},
    title = "Carbon, nitrogen, and oxygen abundances in G8-K3 giant stars",
    journal = {\aap},
    year = 1982,
    month = nov,
    volume = 115,
    pages = {145--163},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1982A%26A...115..145K&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Koechlin1985A&A...153...91K,
    author = {{Koechlin}, L. and {Rabbia}, Y.},
    title = "Stellar diameter measurements with the CERGA optical interferometer - Recent developments and results",
    journal = {\aap},
    year = 1985,
    month = dec,
    volume = 153,
    pages = {91--98},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1985A%26A...153...91K&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Kovacs1983A&A...120...21K,
    author = {{Kov\'{a}cs}, N.},
    title = "{Model-atmosphere analysis of high-dispersion spectra of four red giants and supergiants}",
    journal = {\aap},
    year = 1983,
    month = apr,
    volume = 120,
    pages = {21--35},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1983A%26A...120...21K&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}



@ARTICLE{Kupka1999A&AS..138..119K,
    author = {{Kupka}, F. and {Piskunov}, N. and {Ryabchikova}, T.\ A. and 
        {Stempels}, H.\ C. and {Weiss}, W.\ W.},
    title = {VALD-2: Progress of the Vienna Atomic Line Data Base},
    journal = {\aaps},
    year = 1999,
    month = jul,
    volume = 138,
    pages = {119--133},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1999A%26AS..138..119K&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Kurucz1970SAOSR.308.....K,
    author = {{Kurucz}, R.\ L.},
    title = "Atlas: a Computer Program for Calculating Model Stellar Atmospheres",
    journal = {SAO Special Report},
    year = 1970,
    month = feb,
    volume = 308,
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1970SAOSR.308.....K&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Kurucz1975SAOSR.362.....K,
    author = {{Kurucz}, R.\ L. and {Peytremann}, E.},
    title = {A table of semiempirical gf values.  Part 1: Wavelengths:  5.2682 NM to 272.3380 NM},
    journal = {SAO Special Report},
    year = 1975,
    month = feb,
    volume = 362,
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1975SAOSR.362.....K&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{Kurucz1979ApJS...40....1K,
    author = {{Kurucz}, R.\ L.},
    title = "Model atmospheres for G, F, A, B, and O stars",
    journal = {\apjs},
    year = 1979,
    month = may,
    volume = 40,
    pages = {1 -- 340},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1979ApJS...40....1K&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{Kurucz1979Smith,
        AUTHOR  = {{Kurucz}, R.\ L. and {Furenlid}, I.},
        TITLE   = "",
        YEAR    = 1979,
        JOURNAL = {Smithsonian Astrophys.\ Obs.\ Spec.\ Rept.},
        VOLUME  = {387},
        PAGES   = ""}


@BOOK{Kurucz1989,
        AUTHOR  = "{Kurucz}, R.\ L.",
        TITLE   = "New gf-calculations",
        PUBLISHER = {magnetic tape},
        YEAR    = 1989,
        ADDRESS = ""}

@INPROCEEDINGS{Kurucz1991sabc.conf..441K,
    author = {{Kurucz}, R.\ L.},
    title = "New Opacity Calculations",
    booktitle = {Stellar Atmospheres: Beyond Classical Models, Proceedings of the Advanced Research Workshop.},  
    year = 1991,
    pages = {441},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1991sabc.conf..441K&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Kurucz1992RMxAA..23...45K,
    author = {{Kurucz}, R.\ L.},
    title = "Atomic and Molecular Data for Opacity Calculations",
    journal = {Revista Mexicana de Astronomia y Astrofisica},
    year = 1992,
    month = mar,
    volume = 23,
    pages = {45},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1992RMxAA..23...45K&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Kurucz1993KurCD..13.....K,
    author = {{Kurucz}, R.},
    title = "ATLAS9 Stellar Atmosphere Programs and 2 km/s grid.",
    journal = {ATLAS9 Stellar Atmosphere Programs and 2 km/s grid.\ Kurucz CD-ROM No.\ 13.\  Cambridge, MA: Smithsonian Astrophysical Observatory},
    year = 1993,
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1993KurCD..13.....K&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@BOOK{Kurucz1993sssp.book.....K,
    author = {{Kurucz}, R.\ L.},
    title = "SYNTHE spectrum synthesis programs and line data",
    publisher = {Kurucz CD-ROM, Cambridge, MA: Smithsonian Astrophysical Observatory},
    year = 1993,
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1993sssp.book.....K&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Kyrolainen1986A&AS...65...11K,
    author = {{Kyr\"{o}l\"{a}inen}, J. and {Tuominen}, I. and {Vilhu}, O. and {Virtanen}, H.
        },
    title = "Optical spectroscopy of eleven G- and K-giants",
    journal = {\aaps},
    year = 1986,
    month = jul,
    volume = 65,
    pages = {11--20},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1986A%26AS...65...11K&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{Lambert1976MSRSL...9..405L,
    author = {{Lambert}, D.~L.},
    title = "{The C-12/C-13 ratio in late-type stellar atmospheres}",
    journal = {Memoires of the Societe Royale des Sciences de Liege},
    year = 1976,
    volume = 9,
    pages = {405--415},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1976MSRSL...9..405L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Lambert1980ApJ...235..114L,
    author = {{Lambert}, D.\ L. and {Dominy}, J.\ F. and {Sivertsen}, S.},
    title = "Lithium in late-type giants. I - G and K giants",
    journal = {\apj},
    year = 1980,
    month = jan,
    volume = 235,
    pages = {114--125},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1980ApJ...235..114L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Lambert1981ApJ...248..228L,
    author = {{Lambert}, D.\ L. and {Ries}, L.\ M.},
    title = "Carbon, nitrogen, and oxygen abundances in G and K giants",
    journal = {\apj},
    year = 1981,
    month = aug,
    volume = 248,
    pages = {228--248},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1981ApJ...248..228L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Lambert1982ApJ...254..663L,
    author = {{Lambert}, D.\ L. and {Roby}, S.\ W. and {Bell}, R.\ A.},
    title = "Carbon, nitrogen, and oxygen abundances in Sirius and VEGA",
    journal = {\apj},
    year = 1982,
    month = mar,
    volume = 254,
    pages = {663--669},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1982ApJ...254..663L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Lambert1987Ap&SS.133..369L,
    author = {{Lambert}, D.\ L. and {McWilliam}, A. and {Smith}, V.\ V.},
    title = "Isotopic abundances of silicon in four red giants",
    journal = {\apss},
    year = 1987,
    month = may,
    volume = 133,
    pages = {369--381},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1987Ap%26SS.133..369L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Lamers1994A&A...291..856L,
    author = {{Lamers}, H.\ J.\ G.\ L.\ M. and {Achmad}, L.},
    title = {The relation between microturbulence and mass loss from supergiants},
    journal = {\aap},
    year = 1994,
    month = nov,
    volume = 291,
    pages = {856--868},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1994A%26A...291..856L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Lane1984ApJ...281..723L,
    author = {{Lane}, M.\ C. and {Lester}, J.\ B.},
    title = "Effective temperatures and surface gravities of metallic-line A stars",
    journal = {\apj},
    year = 1984,
    month = jun,
    volume = 281,
    pages = {723--738},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1984ApJ...281..723L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Langhoff1989,
        AUTHOR  = {{Langhoff}, S.\ R. and {Bauschlicher}, C.\ W.\ Jr.},
        TITLE   = { },
        YEAR    = 1989,
        JOURNAL = {J. Chem. Phys.},
        VOLUME  = 91,
        PAGES   = "5953"}

@ARTICLE{Langhoff1993,
        AUTHOR  = {{Langhoff}, S.\ R. and {Bauschlicher}, C.\ W.\ Jr.},
        TITLE   = { },
        YEAR    = 1993,
        JOURNAL = {Chem. Phys. Letters},
        VOLUME  = 211,
        PAGES   = "305"}

@ARTICLE{Lazaro1991MNRAS.249...62L,
    author = {{Lazaro}, C. and {Lynas-Gray}, A.\ E. and {Clegg}, R.\ E.\ S. and 
        {Mountain}, C.\ M. and {Zadrozny}, A.},
    title = "Carbon abundances and isotope ratios in 70 bright M giants",
    journal = {\mnras},
    year = 1991,
    month = mar,
    volume = 249,
    pages = {62--68},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1991MNRAS.249...62L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Lee1970ApJ...162..217L,
    author = {{Lee}, T.~A.},
    title = "{Photometry of high-luminosity M-type stars}",
    journal = {\apj},
    year = 1970,
    month = oct,
    volume = 162,
    pages = {217},
    url = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1970ApJ...162..217L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@INPROCEEDINGS{Leech2002,                                       
        AUTHOR  = "{Leech}, K. and {Kester}, D. and {Shipman}, R. and {Beintema}, D. and {Feuchtgruber}, H. and {Heras}, A. and {Huygen}, R. and {Lahuis}, F. and {Lutz}, D. and {Morris}, P. and {Roelfsema}, P. and {Salama}, A. and {Schaeidt}, S. and {Valentijn}, E. and {Vandenbussche}, B. and {Wieprecht}, E. and {de Graauw} T.", 
        TITLE   = "SWS --- The Short Wavelength Spectrometer",
        BOOKTITLE = "The ISO Handbook. Volume V. SWS - The Short Wavelength 
                     Spectrometer",     
        YEAR    = 2002,
      EDITOR    = "{Leech}, K."}


@ARTICLE{Leggett1986A&A...159..217L,
    author = {{Leggett}, S.\ K. and {Mountain}, C.\ M. and {Selby}, M.\ J. and 
        {Blackwell}, D.\ E. and {Booth}, A.\ J. and {Haddock}, D.\ J. and 
        {Petford}, A.\ D.},
    title = "The effective temperatures, diameters and luminosities of 22 bright stars by application of the infrared flux method",
    journal = {\aap},
    year = 1986,
    month = apr,
    volume = 159,
    pages = {217--222},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1986A%26A...159..217L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Lejeune2001A&A...366..538L,
    author = {{Lejeune}, T. and {Schaerer}, D.},
    title = "{Database of Geneva stellar evolution tracks and isochrones  for (UBV)<SUB>J</SUB>(RI)<SUB>C</SUB> JHKLL'M, HST-WFPC2, Geneva   and Washington photometric systems}",
    journal = {\aap},
    year = 2001,
    month = feb,
    volume = 366,
    pages = {538--546},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2001A%26A...366..538L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}
@ARTICLE{Lemke1990A&A...240..331L,
    author = {{Lemke}, M.},
    title = "Abundance anomalies in main sequence A stars. II - C, Si, CA and the heavy elements SR and BA",
    journal = {\aap},
    year = 1990,
    month = dec,
    volume = 240,
    pages = {331--345},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1990A%26A...240..331L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Lester1986ApJS...61..509L,
    author = {{Lester}, J.\ B. and {Gray}, R.\ O. and {Kurucz}, R.\ L.},
    title = {Theoretical uvby-beta indices},
    journal = {\apjs},
    year = 1986,
    month = jul,
    volume = 61,
    pages = {509--529},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1986ApJS...61..509L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Linsky1978ApJ...220..619L,
    author = {{Linsky}, J.\ L. and {Ayres}, T.\ R.},
    title = {Stellar model chromospheres. VI - Empirical estimates of the chromospheric radiative losses of late-type stars},
    journal = {\apj},
    year = 1978,
    month = mar,
    volume = 220,
    pages = {619--628},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1978ApJ...220..619L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Linsky1979ApJS...41...47L,
    author = {{Linsky}, J.~L. and {McClintock}, W. and {Robertson}, R.~M. and 
        {Worden}, S.~P.},
    title = "{Stellar model chromospheres. X - High-resolution, absolute flux profiles of the CA II H and K lines in stars of spectral types F0-M2}",
    journal = {\apjs},
    year = 1979,
    month = sep,
    volume = 41,
    pages = {47--74},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1979ApJS...41...47L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@BOOK{Lorente1998,
        AUTHOR  = "{Lorente}, R.",
        TITLE   = {Spectral Resolution of SWS AOT 1},
      PUBLISHER = {ISO-SWS online documentation, http://sws.ster.kuleuven.ac.be},
        YEAR    = 1998}


@ARTICLE{Luck1979ApJ...232..797L,
    author = {{Luck}, R.\ E.},
    title = {The chemical compositions of nine southern supergiant stars},
    journal = {\apj},
    year = 1979,
    month = sep,
    volume = 232,
    pages = {797--806},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1979ApJ...232..797L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Luck1985ApJ...298..782L,
    author = {{Luck}, R.\ E. and {Lambert}, D.\ L.},
    title = {Carbon, nitrogen, and oxygen in intermediate-mass supergiants - Is oxygen underabundant?},
    journal = {\apj},
    year = 1985,
    month = nov,
    volume = 298,
    pages = {782--802},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1985ApJ...298..782L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Luck1995AJ....110.2968L,
    author = {{Luck}, R.\ E. and {Challener}, S.\ L.},
    title = "Chemical Abundances for Very Strong-Lined Giants",
    journal = {\aj},
    year = 1995,
    month = dec,
    volume = 110,
    pages = {2968},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1995AJ....110.2968L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@BOOK{Lutz1999,
        AUTHOR  = "{Lutz}, D. and {Feuchtgruber}, H. and {Morfill}, J.",
        TITLE   = {ISO-SWS grating resolution and instrumental profile as
                  measured by the full resolution modes SWS02 and SWS06},
      PUBLISHER = "ISO-SWS online documentation, http://sws.ster.kuleuven.ac.be",
        YEAR    = 1999},

@ARTICLE{Lyubimkov1984Ap.....19..385L,
    author = {{Lyubimkov}, L.\ S. and {Boyarchuk}, A.\ A.},
    title = {Influence of Deviations from Local Thermodynamics Equilibrium on the Determination of Microturbulence in the Atmospheres of F-Type Supergiants},
    journal = {Astrophysics},
    year = 1984,
    volume = 19,
    pages = {385},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1984Ap.....19..385L&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Mackle1975A&AS...19..303M,
    author = {{M{\"a}ckle}, R. and {Griffin}, R. and {Griffin}, R. and {Holweger}, H.
        },
    title = "A model-atmosphere analysis of the spectrum of Arcturus (basic spectroscopic data)",
    journal = {\aaps},
    year = 1975,
    month = mar,
    volume = 19,
    pages = {303},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1975A%26AS...19..303M&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{Malagnini1986A&A...162..140M,
    author = {{Malagnini}, M.\ L. and {Morossi}, C. and {Rossi}, L. and {Kurucz}, R.\ L.
        },
    title = "The empirical BC versus T(eff) scale for non-supergiant O9-G5 stars",
    journal = {\aap},
    year = 1986,
    month = jul,
    volume = 162,
    pages = {140--150},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1986A%26A...162..140M&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Malagnini1990A&AS...85.1015M,
    author = {{Malagnini}, M.\ L. and {Morossi}, C.},
    title = {Accurate absolute luminosities, effective temperatures, radii, masses and surface gravities for a selected sample of field stars},
    journal = {\aaps},
    year = 1990,
    month = nov,
    volume = 85,
    pages = {1015--1019},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1990A%26AS...85.1015M&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Malagnini1997A&A...326..736M,
    author = {{Malagnini}, M.\ L. and {Morossi}, C.},
    title = {Accuracy of effective temperatures of solar chemical composition stars derived from the flux fitting method.},
    journal = {\aap},
    year = 1997,
    month = oct,
    volume = 326,
    pages = {736--740},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1997A%26A...326..736M&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Manduca1979A&AS...36..411M,
    author = {{Manduca}, A.},
    title = "{Infrared Limb-Darkening Coefficients for Late-Type Giant Model Atmospheres}",
    journal = {\aaps},
    year = 1979,
    month = jun,
    volume = 36,
    pages = {411},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1979A%26AS...36..411M&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Manduca1981ApJ...243..883M,
    author = {{Manduca}, A. and {Bell}, R.\ A. and {Gustafsson}, B.},
    title = "The analysis of infrared fluxes of some late-type stars",
    journal = {\apj},
    year = 1981,
    month = feb,
    volume = 243,
    pages = {883--893},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1981ApJ...243..883M&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Mathis1990ARA&A..28...37M,
    author = {{Mathis}, J.~S.},
    title = "{Interstellar dust and extinction}",
    journal = {\araa},
    year = 1990,
    volume = 28,
    pages = {37--70},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1990ARA%26A..28...37M&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Mauron1992A&A...265..711M,
    author = {{Mauron}, N. and {Caux}, E.},
    title = "K I/Na I scattering observations in circumstellar envelopes - Alpha(1) Herculis, Omicron Ceti, TX PISCIUM and Beta Pegasi",
    journal = {\aap},
    year = 1992,
    month = nov,
    volume = 265,
    pages = {711--725},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1992A%26A...265..711M&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Mauron1995A&A...298..869M,
    author = {{Mauron}, N. and {Guilain}, C.},
    title = "NaI and KI scattering in circumstellar envelopes: new detections around giants and the NaI $\{$lambda$\}$5896/KI $\{$lambda$\}$7699 line ratio.",
    journal = {\aap},
    year = 1995,
    month = jun,
    volume = 298,
    pages = {869},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1995A%26A...298..869M&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{McWilliam1990ApJS...74.1075M,
    author = {{McWilliam}, A.},
    title = {High-resolution spectroscopic survey of 671 GK giants. I - Stellar atmosphere parameters and abundances},
    journal = {\apjs},
    year = 1990,
    month = dec,
    volume = 74,
    pages = {1075--1128},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1990ApJS...74.1075M&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Mendoza1967BOTT....4..106M,
    author = {{Mendoza}, E.~E.},
    title = "{UBVRI photometry of southern bright stars}",
    journal = {Boletin de los Observatorios Tonantzintla y Tacubaya},
    year = 1967,
    volume = 4,
    pages = {106},
    url = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1967BOTT....4..106M&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Mendoza1969BOTT....5...57M,
    author = {{Mendoza}, E.~E.},
    title = "{BVRI photometry of 46 southern bright stars}",
    journal = {Boletin de los Observatorios Tonantzintla y Tacubaya},
    year = 1969,
    volume = 5,
    pages = {57},
    url = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1969BOTT....5...57M&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{Melen1995,
        AUTHOR  = "{M\'{e}len}, F. and {Sauval}, A.\ J. and {Grevesse}, N. and
                  {Farmer}, C.\ B. and {Servais}, C. and {Delbouille}, L. and
                  {Roland}, G.",
        TITLE   = "A new analysis of the OH radical spectrum from solar infrared
                  observations", 
        YEAR    = 1995,
        JOURNAL = jmolspec,
        VOLUME  = 174,
        PAGES   = "490--509"}

@BOOK{Mermilliod1986EgUBV.........M,
    author = {{Mermilliod}, J.-C.},
    title = "{Compilation of Eggen's UBV data, transformed to UBV}",
    journal = {Catalogue of Eggen's UBV data.~(1986)},
    year = 1986,
    publisher = {SIMBAD},
    url = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1986EgUBV.........M&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@BOOK{Mihalas,
        AUTHOR  = "{Mihalas}, D.",
        TITLE   = "Stellar Atmospheres",
      PUBLISHER = "W.H. Freeman and Company",
        YEAR    = 1978,
        ADDRESS = ""}



@ARTICLE{Monnier1998ApJ...502..833M,
    author = {{Monnier}, J.\ D. and {Geballe}, T.\ R. and {Danchi}, W.\ C.
        },
    title = {Temporal Variations of Midinfrared Spectra in Late-Type Stars},
    journal = {\apj},
    year = 1998,
    month = aug,
    volume = 502,
    pages = {833},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1998ApJ...502..833M&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Moon1985Ap&SS.117..261M,
    author = {{Moon}, T.},
    title = {Stellar luminosities and radii from uvby-beta photometry},
    journal = {\apss},
    year = 1985,
    month = dec,
    volume = 117,
    pages = {261--270},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1985Ap%26SS.117..261M&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Moon1985MNRAS.217..305M,
    author = {{Moon}, T.\ T. and {Dworetsky}, M.\ M.},
    title = {Grids for the determination of effective temperature and surface gravity of B, A and F stars using uvby-beta photometry},
    journal = {\mnras},
    year = 1985,
    month = nov,
    volume = 217,
    pages = {305--315},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1985MNRAS.217..305M&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Morossi1993A&A...277..173M,
    author = {{Morossi}, C. and {Franchini}, M. and {Malagnini}, M.\ L. and 
        {Kurucz}, R.\ L. and {Buser}, R.},
    title = "Cool Stars - Spectral Energy Distributions and Model Atmosphere Fluxes",
    journal = {\aap},
    year = 1993,
    month = sep,
    volume = 277,
    pages = {173},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1993A%26A...277..173M&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Morton1991ApJS...77..119M,
    author = {{Morton}, D.\ C.},
    title = {Atomic data for resonance absorption lines. I - Wavelengths longward of the Lyman limit},
    journal = {\apjs},
    year = 1991,
    month = sep,
    volume = 77,
    pages = {119--202},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1991ApJS...77..119M&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Morton1992ApJS...81..883M,
    author = {{Morton}, D.\ C.},
    title = {Atomic Data for Resonance Absorption Lines. I. Wavelengths Longward of the Lyman Limit: Erratum},
    journal = {\apjs},
    year = 1992,
    month = aug,
    volume = 81,
    pages = {883},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1992ApJS...81..883M&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Mozurkewich1991AJ....101.2207M,
    author = {{Mozurkewich}, D. and {Johnston}, K.\ J. and {Simon}, R.\ S. and 
        {Bowers}, P.\ F. and {Gaume}, R. and {Hutter}, D.\ J. and {Colavita}, M.\ M. and 
        {Shao}, M. and {Pan}, X.\ P.},
    title = "Angular diameter measurements of stars",
    journal = {\aj},
    year = 1991,
    month = jun,
    volume = 101,
    pages = {2207--2219},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1991AJ....101.2207M&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Napiwotzki1993A&A...268..653N,
    author = {{Napiwotzki}, R. and {Sch\"{o}nberner}, D. and {Wenske}, V.},
    title = {On the determination of effective temperature and surface gravity of B, A, and F stars using Stromgren UVBY beta photometry},
    journal = {\aap},
    year = 1993,
    month = feb,
    volume = 268,
    pages = {653--666},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1993A%26A...268..653N&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{Neuforge1997A&A...328..261N,
    author = {{Neuforge-Verheecke}, C. and {Magain}, P.},
    title = {Spectroscopic analysis of the Alpha Centauri system},
    journal = {\aap},
    year = 1997,
    month = dec,
    volume = 328,
    pages = {261--268},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1997A%26A...328..261N&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Nicolet1978A&AS...34....1N,
    author = {{Nicolet}, B.},
    title = "{Photoelectric photometric catalogue of homogeneous measurements in the UBV system.}",
    journal = {\aaps},
    year = 1978,
    month = oct,
    volume = 34,
    pages = {1--49},
    url = {http://cdsads.u-strasbg.fr/cgi-bin/nph-bib_query?bibcode=1978A%26AS...34....1N&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Oinas1977A&A....61...17O,
    author = {{Oinas}, V.},
    title = "Neutral-ion anomaly in cool stars",
    journal = {\aap},
    year = 1977,
    month = oct,
    volume = 61,
    pages = {17--20},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1977A%26A....61...17O&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}



@ARTICLE{Partridge+Schwenke1995,
        AUTHOR  = "{Partridge}, H. and {Schwenke}, D.\ W.",
        TITLE   = "The determination of an accurate isotope dependent potential
                  energy surface for water from extensive ab initio calculations
                  and experimental data",
        YEAR    = 1997,
        JOURNAL = jchemp,
        VOLUME  = 106,
        PAGES   = "4618--4639"}

@ARTICLE{Pasquini1990A&A...234..277P,
    author = {{Pasquini}, L. and {Brocato}, E. and {Pallavicini}, R.},
    title = "{Chromospheric activity of evolved late-type stars - Chromospheric activity in evolved stars}",
    journal = {\aap},
    year = 1990,
    month = aug,
    volume = 234,
    pages = {277--283},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1990A%26A...234..277P&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Pasquini1992A&A...266..340P,
    author = {{Pasquini}, L. and {Brocato}, E.},
    title = "Chromospheric activity and stellar evolution - Clues from IUE data",
    journal = {\aap},
    year = 1992,
    month = dec,
    volume = 266,
    pages = {340--346},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1992A%26A...266..340P&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Perrin1998A&A...331..619P,
    author = {{Perrin}, G. and {Coude Du Foresto}, V. and {Ridgway}, S.\ T. and 
        {Mariotti}, J.\ -. and {Traub}, W.\ A. and {Carleton}, N.\ P. and 
        {Lacasse}, M.\ G.},
    title = "Extension of the effective temperature scale  of giants to types later than M6",
    journal = {\aap},
    year = 1998,
    month = mar,
    volume = 331,
    pages = {619--626},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1998A%26A...331..619P&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Peterson1993ApJ...404..333P,
    author = {{Peterson}, R.\ C. and {Dalle Ore}, C.\ M. and {Kurucz}, R.\ L.
        },
    title = "The nonsolar abundance ratios of Arcturus deduced from spectrum synthesis",
    journal = {\apj},
    year = 1993,
    month = feb,
    volume = 404,
    pages = {333--347},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1993ApJ...404..333P&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{Pilachowski1997AJ....114..819P,
    author = {{Pilachowski}, C. and {Sneden}, C. and {Hinkle}, K. and {Joyce}, R.
        },
    title = "Carbon Isotope Ratios from the First Overtone CO Bands in Metal-Poor Giants.",
    journal = {\aj},
    year = 1997,
    month = aug,
    volume = 114,
    pages = {819--824},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1997AJ....114..819P&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@INPROCEEDINGS{Piskunov1995lahr.conf..610P,
    author = {{Piskunov}, N.\ E. and {Kupka}, F. and {Ryabchikova}, T.\ A. and 
        {Weiss}, W.\ W. and {Jeffery}, C.\ S.},
    title = {The Vienna Atomic Line Data-Base},
    booktitle = {ASP Conf. Ser. 81: Laboratory and Astronomical High Resolution Spectra},
    year = 1995,
    pages = {610},
     EDITOR    = {{Sauval}, A.\ J. and {Blomme}, R. and {Grevesse}, N.},
        ADDRESS = "ASP"}



@ARTICLE{Plez1992A&A...256..551P ,
    author = {{Plez}, B. and {Brett}, J.\ M. and {Nordlund}, {\AA}.},
    title = {Spherical opacity sampling model atmospheres for M-giants. I - Techniques, data and discussion},
    journal = {\aap},
    year = 1992,
    month = mar,
    volume = 256,
    pages = {551--571},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1992A%26A...256..551P&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Plez1993ApJ...418..812P,
    author = {{Plez}, B. and {Smith}, V.\ V. and {Lambert}, D.\ L.},
    title = {Lithium Abundances and Other Clues to Envelope Burning in Small Magellanic Cloud Asymptotic Giant Branch Stars},
    journal = {\apj},
    year = 1993,
    month = dec,
    volume = 418,
    pages = {812},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1993ApJ...418..812P&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Popper1980ARA&A..18..115P,
    author = {{Popper}, D.~M.},
    title = "{Stellar masses}",
    journal = {\araa},
    year = 1980,
    volume = 18,
    pages = {115--164},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1980ARA%26A..18..115P&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{Popper1993ApJ...404L..67P,
    author = {{Popper}, D.\ M.},
    title = {Main-sequence G and K stellar masses},
    journal = {\apjl},
    year = 1993,
    month = feb,
    volume = 404,
    pages = {L67--L70},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1993ApJ...404L..67P&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Pottasch1992A&A...264..138P,
    author = {{Pottasch}, E.\ M. and {Butcher}, H.\ R. and {van Hoesel}, F.\ H.\ J.
        },
    title = {Solar-like oscillations on Alpha Centauri A},
    journal = {\aap},
    year = 1992,
    month = oct,
    volume = 264,
    pages = {138--146},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1992A%26A...264..138P&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Pourbaix1999A&A...344..172P,
    author = {{Pourbaix}, D. and {Neuforge-Verheecke}, C. and {Noels}, A.},
    title = {Revised masses of alpha  Centauri},
    journal = {\aap},
    year = 1999,
    month = apr,
    volume = 344,
    pages = {172--176},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1999A%26A...344..172P&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Price1968AJ.....73..431P,
    author = {{Price}, S.~D.},
    title = "{Results of an infrared stellar survey.}",
    journal = {\aj},
    year = 1968,
    month = aug,
    volume = 73,
    pages = {431},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1968AJ.....73..431P&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Qiu2001Apj...548...953Q,
    author = {{Qiu}, H.\M. and {Zhao}, G. and {Chen}, Y.\ Q. and {Li}, Z.\ W.},
    title = "The abundance patterns of Sirius and Vega",
    journal = {\aap},
    year = 2001,
    month = feb,
    volume = 548,
    pages = {953--965},
    url = {},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Quirrenbach1993ApJ...406..215Q,
    author = {{Quirrenbach}, A. and {Mozurkewich}, D. and {Armstrong}, J.\ T. and 
        {Buscher}, D.\ F. and {Hummel}, C.\ A.},
    title = "Angular diameter measurements of cool giant stars in strong TiO bands and in the continuum",
    journal = {\apj},
    year = 1993,
    month = mar,
    volume = 406,
    pages = {215--219},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1993ApJ...406..215Q&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}



@ARTICLE{Quirrenbach1996A&A...312..160Q,
    author = {{Quirrenbach}, A. and {Mozurkewich}, D. and {Buscher}, D.\ F. and 
        {Hummel}, C.\ A. and {Armstrong}, J.\ T.},
    title = "Angular diameter and limb darkening of Arcturus.",
    journal = {\aap},
    year = 1996,
    month = aug,
    volume = 312,
    pages = {160--166},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1996A%26A...312..160Q&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Rentzsch-Holm1997A&A...317..178R,
    author = {{Rentzsch-Holm}, I.},
    title = "Abundance anomalies in main sequence A stars. III. Nitrogen and sulphur.", 
    journal = {\aap},
    year = 1997,
    month = jan,
    volume = 317,
    pages = {178--184},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1997A%26A...317..178R&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Ridgway1980ApJ...235..126R,
    author = {{Ridgway}, S.~T. and {Joyce}, R.~R. and {White}, N.~M. and {Wing}, R.~F.
        },
    title = "{Effective temperatures of late-type stars - The field giants from K0 to M6}",
    journal = {\apj},
    year = 1980,
    month = jan,
    volume = 235,
    pages = {126--137},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1980ApJ...235..126R&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@PHDTHESIS{Ries1981,
    author = {{Ries}, L.\ M.},
    title = {Carbon, nitrogen, and oxygen abundances in G and K giants},
    school = {Texas Univ., Arlington.},
    year = 1981,
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1981PhDT.........4R&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Robinson1998ApJ...503..396R,
    author = {{Robinson}, R.\ D. and {Carpenter}, K.\ G. and {Brown}, A.},
    title = "Goddard High-Resolution Spectrograph Observations of Cool Low-Gravity Stars. IV. A Comparison of the K5 III Stars alpha Tauri and gamma Draconis",
    journal = {\apj},
    year = 1998,
    month = aug,
    volume = 503,
    pages = {396},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1998ApJ...503..396R&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Roby1990ApJS...73...67R,
    author = {{Roby}, S.\ W. and {Lambert}, D.\ L.},
    title = "Carbon, nitrogen, and oxygen abundances in the chemically peculiar stars of the upper main sequence",
    journal = {\apjs},
    year = 1990,
    month = may,
    volume = 73,
    pages = {67--0049},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1990ApJS...73...67R&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Rodgers1991ApJ...382..606R,
    author = {{Rodgers}, B. and {Glassgold}, A.\ E.},
    title = "The temperature of the circumstellar envelope of Alpha Orionis",
    journal = {\apj},
    year = 1991,
    month = dec,
    volume = 382,
    pages = {606--616},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1991ApJ...382..606R&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Russell1989ApJS...70..865R,
    author = {{Russell}, S.\ C. and {Bessell}, M.\ S.},
    title = {Abundances of the heavy elements in the Magellanic Clouds. I - Metal abundances of F-type supergiants},
    journal = {\apjs},
    year = 1989,
    month = aug,
    volume = 70,
    pages = {865--898},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1989ApJS...70..865R&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@BOOK{Reader1980wtpa.book.....R,
    author = {{Reader}, J. and {Corliss}, C.\ H. and {Wiese}, W.\ L. and {Martin}, G.\ A.
        },
    title = {Wavelengths and transition probabilities for atoms and atomic ions - Part 1: Wavelengths - Part 2: Transition probabilities},
    publisher = {NSRDS-NBS 68, Washington},
    year = 1980,
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1980wtpa.book.....R&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Relyea1978ApJS...37...45R,
    author = {{Relyea}, L.\ J. and {Kurucz}, R.\ L.},
    title = "A theoretical analysis of UVBY photometry",
    journal = {\apjs},
    year = 1978,
    month = may,
    volume = 37,
    pages = {45--69},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1978ApJS...37...45R&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@PHDTHESIS{Ries1981PhDT.........4R,
    author = {{Ries}, L.\ M.},
    title = "Carbon, nitrogen, and oxygen abundances in G and K giants",
    school = {Texas Univ., Arlington.},
    year = 1981,
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1981PhDT.........4R&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Ryabchikova1997BaltA...6..244R,
    author = {{Ryabchikova}, T.\ A. and {Piskunov}, N.\ E. and {Kupka}, F. and 
        {Weiss}, W.\ W.},
    title = {The Vienna Atomic Line Database : Present State and Future Development},
    journal = {Baltic Astronomy},
    year = 1997,
    month = mar,
    volume = 6,
    pages = {244--247},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1997BaltA...6..244R&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Ryde1999A&A...341..579R,
    author = {{Ryde}, N. and {Eriksson}, K. and {Gustafsson}, B.},
    title = "The nature of the circumstellar CO\_2 emission from M giants",
    journal = {\aap},
    year = 1999,
    month = jan,
    volume = 341,
    pages = {579--586},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1999A%26A...341..579R&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Sadakane1981PASJ...33..189S,
    author = {{Sadakane}, K. and {Nishimura}, M.},
    title = "Metal Abundances and the Microturbulence in VEGA",
    journal = {\pasj},
    year = 1981,
    volume = 33,
    pages = {189},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1981PASJ...33..189S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Sadakane1989PASJ...41..279S,
    author = {{Sadakane}, K. and {Ueta}, M.},
    title = "Abundance analysis of Sirius in the blue-violet region",
    journal = {\pasj},
    year = 1989,
    volume = 41,
    pages = {279--288},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1989PASJ...41..279S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Sanner1976ApJS...32..115S,
    author = {{Sanner}, F.},
    title = "Mass loss in red giants and supergiants",
    journal = {\apjs},
    year = 1976,
    month = sep,
    volume = 32,
    pages = {115--145},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1976ApJS...32..115S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}



@BOOK{Sauval2000,
        AUTHOR  = {{Sauval}, A.\ J.},
        TITLE   = "Data file of IR solar atomic lines",
      PUBLISHER = {unpublished results},
        YEAR    = 2002,
        ADDRESS = ""}


@ARTICLE{Scalo1976ApJ...206..474S,
    author = {{Scalo}, J.~M.},
    title = "{A composite Hertzsprung-Russell diagram for the peculiar red giants}",
    journal = {\apj},
    year = 1976,
    month = jun,
    volume = 206,
    pages = {474--489},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1976ApJ...206..474S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Scalo1978ApJ...225..523S,
    author = {{Scalo}, J.~M. and {Miller}, G.~E.},
    title = "{A constraint on proposed explanations for low $^{12}$C/$^{13}$C ratios in G-K giants}",
    journal = {\apj},
    year = 1978,
    month = oct,
    volume = 225,
    pages = {523--526},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1978ApJ...225..523S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{Scargle1979ApJ...228..838S,
    author = {{Scargle}, J.\ D. and {Strecker}, D.\ W.},
    title = "Cool stars - Effective temperatures, angular diameters, and reddening determined from 1-5 micron flux curves and model atmospheres",
    journal = {\apj},
    year = 1979,
    month = mar,
    volume = 228,
    pages = {838--853},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1979ApJ...228..838S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}



@ARTICLE{Schaeidt1996A&A...315L..55S,
    author = {{Schaeidt}, S.\ G. and {Morris}, P.\ W. and {Salama}, A. and 
        {Vandenbussche}, B. and {Beintema}, D.\ A. and {Boxhoorn}, D.\ R. and 
        {Feuchtgruber}, H. and {Heras}, A.\ M. and {Lahuis}, F. and 
        {Leech}, K. and {Roelfsema}, P.\ R. and {Valentijn}, E.\ A. and 
        {Bauer}, O.\ H. and {van der Bliek}, N.\ S. and {Cohen}, M. and 
        {de Graauw}, T. and {Haser}, L.\ N. and {van der Hucht}, K.\ A. and 
        {Huygen}, E. and {Katterloher}, R.\ O. and {Kessler}, M.\ F. and 
        {Koornneef}, J. and {Luinge}, W. and {Lutz}, D. and {Planck}, M. and 
        {Spoon}, H. and {Waelkens}, C. and {Waters}, L.\ B.\ F.\ M. and 
        {Wieprecht}, E. and {Wildeman}, K.\ J. and {Young}, E. and {Zaal}, P.
        },
    title = {The photometric calibration of the ISO Short Wavelength Spectrometer.},
    journal = {\aap},
    year = 1996,
    month = nov,
    volume = 315,
    pages = {L55--L59},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1996A%26A...315L..55S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@INPROCEEDINGS{Shipman2001clim.confE..18S,
    author = {{Shipman}, R.\ F. and {Morris}, P.\ W. and {Beintema}, D.\ A. and 
        {Boxhoorn}, D. and {Feuchtgruber}, H. and {Heras}, A.\ M. and 
        {Huygen}, R. and {Kester}, D. and {Lahuis}, F. and {Leech}, K. and 
        {Lorente}, R. and {Lutz}, D. and {Roelfsema}, P. and {Salama}, A. and 
        {Schaeidt}, S.\ G. and {Valentijn}, E. and {Vandenbussche}, B. and 
        {Wieprecht}, E.},
    title = "SWS In-flight Calibration",
    booktitle = {`The calibration legacy of the ISO Mission'},
    year = 2001,
    pages = {to be published},
      EDITOR    = {{Metcalfe}, L. and {Kessler}, M.},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2001clim.confE..18S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}





@BOOK{Seaton1995QB809.O63......,
    author = {{Seaton}, M.\ J.},
    title = {The opacity project},
    publisher = {Bristol, UK ; Philadelphia : Institute of Physics Pub.},
    year = 1995,
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1995QB809.O63......&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{Smalley1993A&A...271..515S,
    author = {{Smalley}, B. and {Dworetsky}, M.\ M.},
    title = {The Atmospheric Parameters of A-Stars and F-Stars - Part One - Comparison of Various Methods},
    journal = {\aap},
    year = 1993,
    month = apr,
    volume = 271,
    pages = {515},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1993A%26A...271..515S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Smalley1995A&A...293..446S,
    author = {{Smalley}, B. and {Dworetsky}, M.\ M.},
    title = {The calibration of uvby$\{$beta$\}$ photometry for B, A and F stars. I. Fundamental atmospheric parameters.},
    journal = {\aap},
    year = 1995,
    month = jan,
    volume = 293,
    pages = {446--456},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1995A%26A...293..446S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Smalley1997A&A...328..349S,
    author = {{Smalley}, B. and {Kupka}, F.},
    title = "{The role of convection on the UVBY colours of A, F, and G stars}",
    journal = {\aap},
    year = 1997,
    month = dec,
    volume = 328,
    pages = {349--360},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1997A%26A...328..349S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Smith1985ApJ...294..326S,
    author = {{Smith}, V.\ V. and {Lambert}, D.\ L.},
    title = {The chemical composition of red giants. I - Dredge-up in the M and MS stars},
    journal = {\apj},
    year = 1985,
    month = jul,
    volume = 294,
    pages = {326--338},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1985ApJ...294..326S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Smith1986A&A...165..126S,
    author = {{Smith}, G. and {Edvardsson}, B. and {Frisk}, U.},
    title = "Non-resonance lines of neutral calcium in the spectra of the Alpha Centauri binary system",
    journal = {\aap},
    year = 1986,
    month = sep,
    volume = 165,
    pages = {126--134},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1986A%26A...165..126S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Smith1986ApJ...311..843S,
    author = {{Smith}, V.\ V. and {Lambert}, D.\ L.},
    title = {The chemical composition of red giants. II - Helium burning and the s-process in the MS and S stars},
    journal = {\apj},
    year = 1986,
    month = dec,
    volume = 311,
    pages = {843--863},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1986ApJ...311..843S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Smith1990ApJS...72..387S,
    author = {{Smith}, V.\ V. and {Lambert}, D.\ L.},
    title = "The chemical composition of red giants. III - Further CNO isotopic and s-process abundances in thermally pulsing asymptotic giant branch stars",
    journal = {\apjs},
    year = 1990,
    month = feb,
    volume = 72,
    pages = {387--416},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1990ApJS...72..387S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Smith1993A&A...274..335S,
    author = {{Smith}, K.\ C. and {Dworetsky}, M.\ M.},
    title = "Elemental Abundances in Normal Late B-Stars and Hgmn-Stars from Co-Added IUE Spectra - Part One - Iron Peak Elements",
    journal = {\aap},
    year = 1993,
    month = jul,
    volume = 274,
    pages = {335},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1993A%26A...274..335S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@PHDTHESIS{Sneden1974,
    author = {{Sneden}, C.},
    school = {University of Texas},
    year = 1974,
}


@INPROCEEDINGS{Sneden1991IAUS..145..235S,
    author = {{Sneden}, C.},
    title = "CNO Abundances of Stars Undergoing First Dredge up Mixing",
    booktitle = {IAU Symp. 145: Evolution of Stars: the Photospheric Abundance Connection},
    year = 1991,
    volume = 145,
    pages = {235},
    editor= {{Michaud}, G. and {Tutukov}, A.\ V.},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1991IAUS..145..235S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Soderblom1986A&A...158..273S,
    author = {{Soderblom}, D.\ R.},
    title = {The temperatures of Alpha Centauri A and B},
    journal = {\aap},
    year = 1986,
    month = apr,
    volume = 158,
    pages = {273},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1986A%26A...158..273S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Sokolov1995A&AS..110..553S,
    author = {{Sokolov}, N.\ A.},
    title = {The determination of T\_eff\_ of B, A and F main sequence stars from the continuum between 3200 A and 3600 A.},
    journal = {\aaps},
    year = 1995,
    month = may,
    volume = 110,
    pages = {553},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1995A%26AS..110..553S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Spite1989A&A...210...25S,
    author = {{Spite}, F. and {Spite}, M. and {Francois}, P.},
    title = {Chemical evolution of the Magellanic Clouds. I - Metal abundance in three young supergiants of the Small Cloud},
    journal = {\aap},
    year = 1989,
    month = feb,
    volume = 210,
    pages = {25--34},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1989A%26A...210...25S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Stencel1980ApJS...44..383S,
    author = {{Stencel}, R.\ E. and {Linsky}, J.\ L. and {Mullan}, D.\ J. and 
        {Basri}, G.\ S. and {Worden}, S.\ P.},
    title = "The outer atmospheres of cool stars. VII - High resolution, absolute flux profiles of the MG II H and K lines in stars of spectral types F8 to M5",
    journal = {\apjs},
    year = 1980,
    month = nov,
    volume = 44,
    pages = {383--402},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1980ApJS...44..383S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@BOOK{Sugar1985aeli.book.....S,
    author = {{Sugar}, J. and {Corliss}, C.},
    title = {Atomic energy levels of the iron-period elements: Potassium through Nickel},
    publisher = {Washington: American Chemical Society},
    year = 1985,
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1985aeli.book.....S&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Taylor1999A&AS..134..523T,
    author = {{Taylor}, B.\ J.},
    title = "Catalogs of temperatures and [Fe/H] averages for evolved G and K stars",
    journal = {\aaps},
    year = 1999,
    month = feb,
    volume = 134,
    pages = {523--524},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1999A%26AS..134..523T&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{Tielens1983ApJ...271..702T,
    author = {{Tielens}, A.\ G.\ G.\ M.},
    title = "Stationary flows in the circumstellar envelopes of M giants",
    journal = {\apj},
    year = 1983,
    month = aug,
    volume = 271,
    pages = {702--716},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1983ApJ...271..702T&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Tipping1981,
        AUTHOR  = {{Tipping}, R.\ H. and {Chackerian}, C.\ Jr.},
        TITLE   = "",
        YEAR    = 1981,
        JOURNAL = {J.\ Mol. Spectr.},
        VOLUME  = 88,
        PAGES   = "352"}


@ARTICLE{Tomkin1975ApJ...199..436T,
    author = {{Tomkin}, J. and {Lambert}, D.\ L. and {Luck}, R.\ E.},
    title = "The C-12/C-13 ratio in stellar atmospheres. IV - Eleven G and K type giants",
    journal = {\apj},
    year = 1975,
    month = jul,
    volume = 199,
    pages = {436--442},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1975ApJ...199..436T&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Tomkin1976ApJ...210..694T,
    author = {{Tomkin}, J. and {Luck}, R.\ E. and {Lambert}, D.\ L.},
    title = "The 12C/13C ratio in stellar atmospheres. VII. 38 giants and supergiants.",
    journal = {\apj},
    year = 1976,
    month = dec,
    volume = 210,
    pages = {694--701},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1976ApJ...210..694T&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Trimble1981QJRAS..22..361T,
    author = {{Trimble}, V. and {Bell}, R.\ A.},
    title = {Spectroscopic Determination of Stellar Masses - Mene Tekel Arcturus},
    journal = {\qjras},
    year = 1981,
    volume = 22,
    pages = {361},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1981QJRAS..22..361T&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Tsuji1981A&A....99...48T,
    author = {{Tsuji}, T.},
    title = {Spectral energy distribution and effective temperature scale of M-giant stars. II - Application of the infra-red flux method},
    journal = {\aap},
    year = 1981,
    month = jun,
    volume = 99,
    pages = {48--57},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1981A%26A....99...48T&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{Tsuji1986A&A...156....8T,
    author = {{Tsuji}, T.},
    title = "High resolution spectroscopy of CO in the infrared spectra of cool stars - Turbulent velocities and carbon abundance in M-giant stars",
    journal = {\aap},
    year = 1986,
    month = feb,
    volume = 156,
    pages = {8--21},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1986A%26A...156....8T&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Tsuji1991A&A...245..203T,
    author = {{Tsuji}, T.},
    title = "High resolution spectroscopy of CO in the infrared spectra of cool stars. III - Line intensities, shifts, and asymmetries as probes of stellar turbulence and abundance in oxygen-rich giants",
    journal = {\aap},
    year = 1991,
    month = may,
    volume = 245,
    pages = {203--218},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1991A%26A...245..203T&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{Tsuji1994A&A...289..469T,
    author = {{Tsuji}, T. and {Ohnaka}, K. and {Hinkle}, K.\ H. and {Ridgway}, S.\ T.
        },
    title = "High resolution infrared spectra of silicon monoxide and silicon isotopic abundances in cool luminous stars",
    journal = {\aap},
    year = 1994,
    month = sep,
    volume = 289,
    pages = {469--491},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1994A%26A...289..469T&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Tsuji1997A&A...320L...1T,
    author = {{Tsuji}, T. and {Ohnaka}, K. and {Aoki}, W. and {Yamamura}, I.
        },
    title = {Warm molecular envelope of M giants and Miras: a new molecule forming region unmasked by the ISO SWS.},
    journal = {\aap},
    year = 1997,
    month = apr,
    volume = 320,
    pages = {L1--L4},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1997A%26A...320L...1T&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@BOOK{Vandenbussche1999,
        AUTHOR  = "{Vandenbussche}, B.",
        TITLE   = {The ISO-SWS Relative Spectral Response Calibration},
      PUBLISHER = {ISO-SWS online documentation},
        YEAR    = 1999}



@INPROCEEDINGS{Vandenbussche2001clim.confE..97V,
    author = {{Vandenbussche}, B. and {Morris}, P.~W. and {Valentijn}, E.~A. and 
        {Beintema}, D.~A. and {Boxhoorn}, D.~R. and {Decin}, L. and 
        {Feuchtgruber}, H. and {Heras}, A.~M. and {Lahuis}, F. and {Lorente}, R. and 
        {Lutz}, D. and {Roelfsema}, P.~R. and {Salama}, A. and {Schaeidt}, S.~G. and 
        {Shipman}, R.~F. and {Spoon}, H.~W.~W. and {van Malderen}, R. and 
        {Waters}, L.~B.~F.~M. and {Wieprecht}, E. and {Zaal}, P.},
    title = "{The Relative Spectral Response Calibration of the ISO-SWS}",
    booktitle = {The Calibration Legacy of the ISO Mission},
    year = 2001,
    pages = {97},
      EDITOR    = {{Metcalfe}, L. and {Kessler}, M.},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=2001clim.confE..97V&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@INPROCEEDINGS{Vanhoof1998sese.conf...67V,
    author = {{van Hoof}, P.\ A.\ M.},
    title = {A comprehensive line list for atomic transitions on the WWW},
    booktitle = {Stellar Evolution, Stellar Explosions and Galactic Chemical Evolution},
    year = 1998,
    pages = {67},
      EDITOR    = {{Mezzacappa}, A.},
        ADDRESS = "Institute of Physics Publishing"}

@ARTICLE{vanParadijs1973A&A....23..369V,
    author = {{van Paradijs}, J.},
    title = "An analysis of the line spectra of some G and K Ib supergiants.",
    journal = {\aap},
    year = 1973,
    month = mar,
    volume = 23,
    pages = {369},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1973A%26A....23..369V&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{vanParadijs1974A&A....35..225V,
    author = {{van Paradijs}, J. and {Meurs}, E.\ J.\ A.},
    title = "A differential abundance analysis of alpha Tau relative to alpha Boo",
    journal = {\aap},
    year = 1974,
    month = oct,
    volume = 35,
    pages = {225--231},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1974A%26A....35..225V&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{vanParadijs1976A&A....53....1V,
    author = {{van Paradijs}, J. and {Kester}, D.},
    title = "{Abondances of carbon, nitrogen and oxygen in six G and K type giants.}",
    journal = {\aap},
    year = 1976,
    month = nov,
    volume = 53,
    pages = {1--8},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1976A%26A....53....1V&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}


@ARTICLE{Venn1990ApJ...363..234V,
    author = {{Venn}, K.\ A. and {Lambert}, D.\ L.},
    title = "The chemical composition of three Lambda Bootis stars",
    journal = {\apj},
    year = 1990,
    month = nov,
    volume = 363,
    pages = {234--244},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1990ApJ...363..234V&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Volk1989AJ.....98.1918V,
    author = {{Volk}, K. and {Cohen}, M.},
    title = {On the calibration of the IRAS low-resolution spectra},
    journal = {\aj},
    year = 1989,
    month = nov,
    volume = 98,
    pages = {1918--1934},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1989AJ.....98.1918V&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Wallace1995Sci...268.1155W,
    author = {{Wallace}, L. and {Bernath}, P. and {Livingston}, W. and {Hinkle}, K. and 
        {Busler}, J. and {Guo}, B. and {Zhang}, K.},
    title = "Water on the Sun",
    journal = {Science},
    year = 1995,
    month = may,
    volume = 268,
    pages = {1155},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1995Sci...268.1155W&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Wamsteker1981A&A....97..329W,
    author = {{Wamsteker}, W.},
    title = "{Standard stars and calibration for JHKLM photometry}",
    journal = {\aap},
    year = 1981,
    month = apr,
    volume = 97,
    pages = {329--333},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1981A%26A....97..329W&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@BOOK{Wiese1966atp..book.....W,
    author = {{Wiese}, W.\ L. and {Smith}, M.\ W. and {Glennon}, B.\ M.},
    title = {Atomic transition probabilities. Vol.: Hydrogen through Neon. A critical data compilation},
    publisher = {NSRDS-NBS 4, Washington},
    year = 1966,
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1966atp..book.....W&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@BOOK{Wiese1969atp..book.....W,
    author = {{Wiese}, W.\ L. and {Smith}, M.\ W. and {Miles}, B.\ M.},
    title = {Atomic transition probabilities. Vol. 2: Sodium through Calcium. A critical data compilation},
    publisher = {NSRDS-NBS 22, Washington},
    year = 1969,
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1969atp..book.....W&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Wilson1976ApJ...205..823W,
    author = {{Wilson}, O.~C.},
    title = "{Absolute magnitudes of stars from widths of chromospheric CaII emission lines.}",
    journal = {\apj},
    year = 1976,
    month = may,
    volume = 205,
    pages = {823--840},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1976ApJ...205..823W&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Witteborn1999AJ....117.2552W,
    author = {{Witteborn}, F.\ C. and {Cohen}, M. and {Bregman}, J.\ D. and 
        {Wooden}, D.\ H. and {Heere}, K. and {Shirley}, E.\ L.},
    title = {Spectral Irradiance Calibration in the Infrared. XI. Comparison of alpha Bootis and 1 Ceres with a Laboratory Standard},
    journal = {\aj},
    year = 1999,
    month = may,
    volume = 117,
    pages = {2552--2560},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1999AJ....117.2552W&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Woitke1999A&A...348L..17W,
    author = {{Woitke}, P. and {Helling}, C. and {Winters}, J.\ M. and {Jeong}, K.\ S.
        },
    title = "On the formation of it warm molecular layers",
    journal = {\aap},
    year = 1999,
    month = aug,
    volume = 348,
    pages = {L17--L20},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1999A%26A...348L..17W&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Worthey1994ApJS...95..107W,
    author = {{Worthey}, G.},
    title = "Comprehensive stellar population models and the disentanglement of age and metallicity effects",
    journal = {\apjs},
    year = 1994,
    month = nov,
    volume = 95,
    pages = {107--149},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1994ApJS...95..107W&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Worthey1994ApJS...94..687W,
    author = {{Worthey}, G. and {Faber}, S.~M. and {Gonzalez}, J.~J. and {Burstein}, D.
        },
    title = "{Old stellar populations. 5: Absorption feature indices for the complete LICK/IDS sample of stars}",
    journal = {\apjs},
    year = 1994,
    month = oct,
    volume = 94,
    pages = {687--722},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1994ApJS...94..687W&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Yamamura1999A&A...341L...9Y,
    author = {{Yamamura}, I. and {de Jong}, T. and {Onaka}, T. and {Cami}, J. and 
        {Waters}, L.\ B.\ F.\ M.},
    title = "Detection of warm SO\_2 gas in oxygen-rich AGB stars",
    journal = {\aap},
    year = 1999,
    month = jan,
    volume = 341,
    pages = {L9--L12},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1999A%26A...341L...9Y&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}

@ARTICLE{Zahn1992A&A...265..115Z,
    author = {{Zahn}, J.\ -.},
    title = "Circulation and turbulence in rotating stars",
    journal = {\aap},
    year = 1992,
    month = nov,
    volume = 265,
    pages = {115--132},
    url = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1992A%26A...265..115Z&db_key=AST},
    adsnote = {Provided by the NASA Astrophysics Data System}
}



